Monoidal weak omega-categories as models of a type theory

Weak $\omega$-categories are notoriously difficult to define because of the very intricate nature of their axioms. Various approaches have been explored, based on different shapes given to the cells. Interestingly, homotopy type theory encompasses a definition of weak $\omega$-groupoid in a globular setting, since every type carries such a structure. Starting from this remark, Brunerie could extract this definition of globular weak $\omega$\nobreakdash-groupoids, formulated as a type theory. By refining its rules, Finster and Mimram have then defined a type theory called CaTT, whose models are weak $\omega$-categories. Here, we generalize this approach to monoidal weak $\omega$-categories. Based on the principle that they should be equivalent to weak $\omega$-categories with only one $0$-cell, we are able to derive a type theory MCaTT whose models are monoidal categories. This requires changing the rules of the theory in order to encode the information carried by the unique $0$-cell. The correctness of the resulting type theory is shown by defining a pair of translations between our type theory MCaTT and the type theory CaTT. Our main contribution is to show that these translations relate the models of our type theory to the models of the type theory CaTT consisting of $\omega$-categories with only one $0$-cell, by analyzing in details how the notion of models interact with the structural rules of both type theories.

==> correctness.tex <==
\section{Correctness}
\label{sec:correctness}
We now prove that $\MCaTT$ is the internal language for monoidal weak
$\omega$\nobreakdash-ca\-te\-go\-ries. Our strategy relies on
the fact that $\CaTT$ is the internal language for weak $\omega$-categories,
establishes a translation between $\MCaTT$ and a restriction of the theory
$\CaTT$ such that all contexts contain exactly $0$-cell. This is made formal
by constructing a pair of functors from the syntactic category of $\MCaTT$ to a
subcategory of the syntactic category of $\CaTT$. Although these translations
require some care in order to ensure that they are properly defined, they merely
formalize our initial intuition behind $\MCaTT$ and most of the proofs are
technical but simple mutual inductions on the structure of the type theory. Our
main contribution is to show how these translations give the expected
equivalence, by analyzing their interaction with the structure of category with
families of the syntactic categories on each side.

\subsection{Translation for pasting schemes}
We now define the operation that formalizes the combinatorial
equivalence between monoidal ps-contexts and ps-contexts shifted in
dimension.


\paragraph{Flattening of monoidal ps-contexts.}
Intuitively, given a monoidal ps-context $\overline\Gamma$ the
operation we define generates a ps-context, by connecting all the
components of $\Gbar$ through a new variable. Later on, the full
translation will identify all the newly introduced variables to end up
in a context with only one object. In order to perform this
translation, we need first to pick an inifnite sequence of fresh
variable names $x_0,x_1,\ldots$ to be used (which can always be done
since proofs are finite and the set of variables is supposed to be
infinite countable). We then define the operation of \emph{flattening}
by mutual induction on monoidal ps-contexts and types containing only
variables:
\begin{align*}
  \bra{}^\flat&= (x_0:\Obj)
  \\
  \bra{\overline\Gamma;\emptycontext}^\flat
              &= (\overline\Gamma^\flat, x_{k+1}: \Obj)
              &
                \bra{\overline{\Gamma};(\Delta,y:A)}^\flat
              &=  \pa{\bra{\overline\Gamma;\Delta}^\flat,y:\Susp[k,k+1] A}
                \intertext{for contexts, with $k = \ell(\overline\Gamma)$, and for types}
                \Susp[n,m]{\Obj\phantom{}}
              &= \Hom\Obj{x_n}{x_m}
              &
                \Susp[n,m]{\Hom {A}xy} &= \Hom{\Susp[n,m]A}xy
\end{align*}
In order to prove that this operation respects ps-contexts, we show
\begin{lemma}
  The two following statements are verified
  \begin{enumerate}
  \item if $\Gbar\vdashps$ then
    $\Gbar^\flat\vdashps x_{\ell(\Gbar)}:\Obj$
  \item if $\Gbar\vdashps$ and $\Delta\vdashps y:A$ then
    $\bra{\Gbar;\Delta}^\flat\vdashps
    y:\Susp[\ell(\Gbar),\ell(\Gbar)+1]A$
  \end{enumerate}
\end{lemma}
\begin{proof}
  These two statements are proved by mutual induction on monoidal
  ps-contexts and types containing only variables.
  \begin{enumerate}
  \item We prove this statement by induction over the list structure
    of monoidal ps-contexts.
    \begin{itemize}
    \item First note that for the monoidal ps-context $\bra{}$, we
      have $\bra{}^\flat = (x_0 : \Obj)$ which satisfies
      indeed$ (x_0 : \Obj) \vdashps x_0 : \Obj $.
    \item Suppose that a monoidal ps-context is of the form
      $\bra{\Gbar;\Delta}$. Then necessarily, this implies
      $\Gbar\vdashps$ and $\Delta\vdashps$, and thus there is a
      judgment of the form $\Delta\vdashps y:\Obj$. By induction, this
      implies that
      $\bra{\Gbar;\Delta}^\flat\vdashps \Hom
      \Obj{x_{\ell(\Gbar)}}{x_{\ell(\Gbar) + 1}}$. By the rule
      \regle{psd}, this
      proves the derivability of $\bra{\Gbar;\Delta}^\flat \vdashps x_{\ell(\Gbar)+ 1} :
      \Obj $.
    \end{itemize}
  \item Fix a monoidal ps-context $\overline\Gamma$ and denote $k$ its
    length, we prove this statement by induction over the structure of
    ps-context.
    \begin{itemize}
    \item For a ps-context of the form $(y:\Obj)\vdashps y:\Obj$, we
      have that
      \[\bra{\Gbar;(y:\Obj)}^\flat = (\Gbar,x_{k + 1} : \Obj,
        y:\Hom{\Obj}{x_{k}}{x_{k + 1}})\] and since by induction we
      have that $\Gbar^\flat\vdashps x_{k} : \Obj$, this proves by
      application of the rule \regle{pse} that
      \[
        \bra{\Gbar;(y:\Obj)}^\flat\vdashps
        y:\Susp[k,k+1]{\Obj\phantom{}}
      \]
    
    \item For a ps-context of the form
      $(\Delta,z:A,f:\Hom Ayz)\vdashps z : \Hom Ayz$ assuming that we
      have $\Delta\vdash y : A$, we have that
      \[
        \bra{\Gbar;(\Delta,z:A,f:\Hom Ayz)}^\flat =
        \pa{\bra{\Gbar;\Delta}^\flat,z:\Susp[k,k+1]A,
          f:\Hom{\Susp[k,k+1]A}yz}
      \]
      and since by induction, we have
      $\bra{\Gbar;\Delta}^\flat\vdashps y:\Susp[k,k+1]A$, it follows by
      application of the rule \regle{pse} that
      \[
        \bra{\Gbar;(\Delta,z:A,f:\Hom Ayz)}^\flat \vdashps f :
        \Susp[k,k+1]{\Hom Ayz}
      \]
    \item For a ps-context of the form $\Delta \vdashps z:A$, assuming
      that we have $\Delta\vdashps f:\Hom Ayz$, by induction we have
      that
      \[
        \bra{\Gbar;\Delta}^\flat\vdashps f:\Hom{\Susp[k,k+1]A}yz
      \]
      and thus by application of the rule \regle{psd}, this proves
      that
      \[
        \bra{\Gbar;\Delta}^\flat\vdashps z:\Susp[k,k+1]A\qedhere
      \]
    \end{itemize}
  \end{enumerate}

    
\end{proof}
\begin{prop}
  \label{prop:ps-flatten-wd}
  The falttening operation sends monoidal ps-contexts in $\MCaTT$ onto
  ps-contexts in $\CaTT$: $\Gbar\vdashps$ implies
  $\Gbar^\flat\vdashps$.
\end{prop}
\begin{proof}
  By the previous lemma, if we have $\Gbar\vdashps$, then we also have
  $\Gbar^\flat\vdashps x_{\ell(\Gbar)} : \Obj$. So, by application of
  the rule \regle{ps}, this proves that $\Gbar^\flat\vdashps$.
\end{proof}

% \begin{notations}
%   This justifies the following choice of notation, which sends a
%   derivable contractibility judgment in $\MCaTT$ to a derivable
%   contractibility judgment in $\CaTT$:
%   \begin{align*}
%     \pa{\overline\Gamma\vdashps}^\flat &= \overline{\Gamma}^\flat\vdashps \\
%     \pa{\overline\Gamma \vdash A}^\flat &= \overline\Gamma^\flat \vdash A^\flat_{0,\ell({\overline{\Gamma}})} \\
%     \pa{\overline\Gamma \vdash t:A}^\flat &= \overline\Gamma^\flat \vdash t_{0,\ell(\Gamma)}^\flat : A^\flat_{0,\ell({\overline{\Gamma}})} \\
%     \pa{\overline\Gamma \vdash \overline\sigma:\overline{\Delta}}^\flat &= \overline\Gamma^\flat \vdash \overline\sigma^\flat_{0,\ell(\Gamma)}:\overline\Delta^\flat\\
%   \end{align*}
% \end{notations}


\paragraph{Folding of a ps-context.}
We now define the operation that goes the opposite way: Given a
ps-context in $\CaTT$, we shift its dimension by $-1$, and remove all
objects of dimension $-1$ to define a monoidal ps-context.  In order
to properly define this operation we introduce the notation
\[
  (\overline{\Gamma},(x:A)) \quad \text{is the list $\overline\Gamma$
    with its last context extended with $(x:A)$}
\]
We call this operation \emph{folding}, and denote it with
$\_^\sharp$. It is defined on contexts as follows
\begin{align*}
  \emptycontext &=  \bra{}
  &
    (\Gamma,x:\Obj) &= \bra{\Gamma^\sharp;\emptycontext}
  &
    (\Gamma,x:A) &= (\Gamma^\sharp,x:A^-) \\
                && \pa{\Hom \Obj xy}^- &= \Obj & \pa{\Hom Axy}^-&= \Hom{A^-}xy  
\end{align*}
Note that there is no case for the type $\Obj$, and this is
intentional since it becomes in $\MCaTT$ the virtual object, that
should never be referred to. This lack of translation for the type
$\Obj$ is very important and manifests itslef throughout our
comparison between the two theories.

\begin{prop}
  \label{prop:ps-fold-wd}
  The folding operation sends ps-contexts onto monoidal ps
  contexts. More precisely, we have the two following statements
  \begin{enumerate}
  \item If $\Gamma\vdashps x:A$ with $A$ distinct from $\Obj$, then
    necessarily $\Gamma^\sharp$ is of the form $\bra{\Gbar;\Delta}$,
    with $\Gbar\vdashps$ and $\Delta\vdashps x:A^-$.
  \item If $\Gamma\vdashps$ then $\Gamma^\sharp\vdashps$.
  \end{enumerate}
\end{prop}
\begin{proof}
  We prove these two statements by induction. The second one is a
  consequence of the first one and one of the induction cases of the
  first one uses the second one.
  \begin{enumerate}
  \item We prove this result by induction on the structure of
    ps-context.
    \begin{itemize}
    \item Here we prevent the type $A$ to be $\Obj$, so the base case
      is actually the case of the context of a derivation of the form
      \[
        (\Gamma,y:\Obj,f:\Hom\Obj xy)\vdashps f:\Hom\Obj xy
      \]
      assuming that $\Gamma \vdashps x:\Obj$. Then by the rule
      \regle{ps}, we also have $\Gamma\vdashps$, and thus by induction
      $\Gamma^\sharp\vdashps$. Moreover, we also have that
      $(f:\Obj)\vdashps f:\Obj$, hence the expected result
      \[
        (\Gamma,y:\Obj,f:\Hom\Obj xy)^\sharp =
        \bra{\Gamma^\sharp;(f:\Obj)} \quad \text{with $\left\{
            \begin{array}{r@{\ }l}
              \Gbar&\vdashps \\
              f:\Obj&\vdashps f:\Obj
            \end{array}
          \right.$}
      \]
    \item In the case of a derivation of the form
      \[
        (\Gamma,y:A,f:\Hom Axy)\vdashps f:\Hom Axy
      \]
      assuming $\Gamma\vdashps x:A$ and $A$ distinct from $\Obj$, we
      have by induction that $\Gamma^\sharp$ is of the form
      $\bra{\Gbar;\Delta}$ with $\Gbar\vdashps$ and
      $\Delta\vdashps x:A^-$. By application of the rule \regle{pse}
      for $\Delta$, we have that
      \[
        (\Delta,y:A^-,f:\Hom{A^-}xy)\vdashps f:\Hom{A^-}xy
      \]
      This proves that
      \begin{align*}
        &(\Gamma,y:A,f:\Hom Axy)^\sharp =
          \bra{\Gbar;(\Delta,y:A^-,f:\Hom{A^-}xy)} \\
        &\qquad\text{with
          $\left\{
          \begin{array}{l}
            \Gbar\vdashps \\
            (\Delta,y:A^-,f:\Hom{A^-}xy)\vdashps f:\Hom{A^-}xy
          \end{array}
        \right.$}
      \end{align*}
    \item In the case of a derivation of the form
      $\Gamma\vdashps y:A$, assuming $\Gamma\vdashps f:\Hom Axy$ with
      $A$ distinct of the type $\Obj$, we have by induction that
      $\Gamma^\sharp$ is of the form $\bra{\Gbar,\Delta}$ with
      $\Gbar\vdashps$ and $\Delta\vdashps f:\Hom{A^-}xy$. By applying
      the rule \regle{psd} to $\Delta$, this proves that
      $\Delta\vdashps y:A^-$, and thus
      \begin{align*}
        \Gamma^\sharp =
        \bra{\Gbar;\Delta} \qquad\text{with
        $\left\{
        \begin{array}{r@{\ }l}
          \Gbar&\vdashps \\
          \Delta&\vdashps y:A^-
        \end{array}
                  \right.$}
      \end{align*}      
    \end{itemize}
  
  \item First note that if $\Gamma$ is the ps-context obtained by a
    unique point: $\Gamma = (x:\Obj)$, then we have
    $\Gamma^\sharp = \bra{}$, and hence $ \Gamma^\sharp\vdashps$.  So
    it suffices to check this property for a ps-context $\Gamma$ which
    is not just one point. For such a ps-context the judgment
    $\Gamma\vdashps$ necessarily comes from a judgment
    $\Gamma\vdashps y:\Obj$, which in turns has to come from a
    judgment of the form $\Gamma\vdashps f:\Hom\Obj yz$. By the
    previous lemma, this proves that $\Gamma^\sharp$ is of the form
    $\bra{\Gbar;\Delta}$, with $\Gbar\vdashps$ and
    $\Delta\vdashps f : \pa{\Hom \Obj yz}^- = \Obj$. By application of
    the rule \regle{ps} on $\Delta$, this proves that
    $\Delta\vdashps$, and thus \[
      \Gamma^\sharp = \bra{\overline\Gamma;\Delta} \vdashps\qedhere\]
  \end{enumerate}
\end{proof}
\noindent
Note that in fact only the second statement is of interest for us, the
first one should be seen as a auxialiary lemma that is mutually
inductive with it and allows for a proof.

\paragraph{Interaction of flattening and folding.}
As the notations suggest, the flattening and folding operations are
inverse to one another. Although this is not true on the nose in one
of the directions, due to the fact that the flattening introduces
fresh variables, it is holds up to renaming of those variables. In
order to prove this, we first prove the following lemma concerning the
action on types with only variables.
\begin{lemma}
  The transformations that we have introduced on types cancel each
  other.
  \begin{enumerate}
  \item For any type $A$ with only variables, we have that
    $\pa{\Susp A}^- = A$
  \item For any type $A$ with only variables and distinct from the the
    type $\Obj$, $\Susp{A^-} = A$ up to renaming of the variables of
    type $\Obj$
  \end{enumerate}
\end{lemma}
\begin{proof}
  These statements are both proved by induction on the structure of
  the types
  \begin{enumerate}
  \item For the type $\Obj$, we have that
    \[
      \pa{\Susp{\Obj}}^- = \pa{\Hom \Obj{x_n}{x_m}}^- = \Obj
    \]
    And for a type of the form $\Hom Axy$, we have that
    \[
      \pa{\Susp{\Hom Axy}}^- = \Hom{\pa{\Susp A}^-}xy
    \]
    By induction this proves the equality.
  \item For a type of the form $\Hom \Obj xy$, we have that
    \[
      \Susp{\pa{\Hom \Obj xy}^-} = \Susp \Obj = \Hom{\Obj}{x_n}{x_m}
    \]
    And for a type of the form $\Hom Axy$, we have that
    \[
      \Susp{\pa{\Hom Axy}}^- = \Hom{\Susp {A^-}}xy
    \]
    By induction this proves the equality up to renaming of the
    variables of type $\Obj$.
    
  \end{enumerate}
\end{proof}

\begin{prop}
  \label{prop:ps-flatten-fold}
  The flattening and folding operations are inverse to one another
  \begin{enumerate}
  \item If $\Gbar\vdashps$, then $\pa{\Gbar^\flat}^\sharp = \Gbar$
  \item If $\Gamma\vdashps$, then $\pa{\Gamma^\sharp}^\flat = \Gamma$
    up to renaming of the variables of type $\Obj$
  \end{enumerate}
\end{prop}
\begin{proof}
  These two statements are both proved by induction
  \begin{enumerate}
  \item We prove this by induction on the structure of lists of
    contexts
    \begin{itemize}
    \item For the monoidal ps-context $\bra{}$, we have that
      \[
        \pa{\bra{}^\flat}^\sharp = (x_0:\Obj)^\sharp = \bra{}
      \]
    \item For a list of contexts of the form
      $\bra{\Gbar;\emptycontext}$, we have
      \[
        \pa{\bra{\Gbar;\emptycontext}^\flat}^\sharp = \pa{\Gbar^\flat,
          x_{\ell(\Gbar)}:\Obj}^\sharp = \pa{\Gbar^\flat}^\sharp =
        \Gbar
      \]
    \item For a list of context of the form
      $\bra{\Gbar;(\Delta,y:A)}$, we have
      \begin{align*}
        \pa{\bra{\Gbar;(\Delta,y:A)}^\flat}^\sharp
        &=
          \pa{\bra{\Gbar;\Delta}^\flat, y : \Susp A}^\sharp\\
        &
          =
          \pa{\pa{\bra{\Gbar;\Delta}^\flat}^\sharp,y:(\Susp A)^- } \\
        &=
          \pa{\bra{\Gbar;\Delta},y:A}\\
        &= \bra{\Gbar;(\Delta,y:A)}       
      \end{align*}
      the penultimate step is obtained by induction and applying the
      previous lemma.
    \end{itemize}
  \item We prove this statement by induction on the structure of
    context
    \begin{itemize}
    \item Since a ps-context is never empty, we do the induction case
      on the context $(y:\Obj)$. We then have
      \[
        \pa{(y:\Obj)^\sharp}^\flat = []^\flat = (x_0:\Obj)
      \]
      So the two contexts are indeed equal up to the renaming of the
      variable.
    \item For a context of the form $(\Gamma,y:\Obj)$, we have that
      \[
        \pa{(\Gamma,y:\Obj)^\sharp}^\flat =
        \bra{\Gamma^\sharp;\emptycontext}^\flat =
        \pa{\pa{\Gamma^\sharp}^\flat,x_{\ell(\Gamma^\sharp)+1} : \Obj}
      \]
      By induction, this is equal to $(\Gamma,y:\Obj)$ up to renaming
      of the variables of type $\Obj$.
    \item For a context of the form $(\Gamma,y:A)$, we have that
      \[
        \pa{(\Gamma,y:A)^\sharp}^\flat =
        \bra{(\Gamma^\sharp,y:A^-)}^\flat =
        \pa{\pa{\Gamma^\sharp}^\flat,y : \Susp{A^-}}
      \]
      By induction and by the previous lemma, this is equal to
      $(\Gamma,y:A)$ up to renaming of the variables of type
      $\Obj$.\qedhere
    \end{itemize}
  \end{enumerate}
\end{proof}


\subsection{Translations for the structure in pasting schemes}
% We now extend these translations back and forth to the types, the
% terms and the substitutions, restricting ourselves to the monoidal
% ps-contexts and the ps-contexts. The definitions of these
% translations are guided by the actions on contexts we just describe.
We have defined a pair of translations back and forth between the
monoidal ps-contexts and the ps-contexts, proving that they are
equivalent. We now show that these translations extend to the types,
terms and substitutions associated to those.

\paragraph{Flattening.}
In order to be consistent with the shift in dimension occurring while
flattening a monoidal ps-context, we define the flattening to shift
dimensions of types, terms and substitutions as well. This is done by
replacing the type $\Obj$ by an arrow and propagating this change by
induction, to types, terms and substitutions. We again use a family of
fresh variables $x_0,x_1,\ldots$, and always replace the type $\Obj$
by an arrow between two of these fresh variables. In order to know
which of these variables should be used, we carry indices.
\[
  \begin{array}{c@{\qquad}l}
    \Obj^\flat_{n,m} = \Hom{}{x_n}{x_m}
    &
      \multicolumn{1}{c}{\pa{\Hom Atu}^\flat_{n,m} = \Hom {A^\flat_{n,m}}{t^\flat_{n,m}}{u^\flat_{n,m}}}
    \\[1.2em]
    \pa{x}^\flat_{n,m} = x
    &
      \multicolumn{1}{c}{\pa{\coh_{\overline\Gamma,A}[\overline\sigma]}^\flat_{n,m} = \coh_{\overline\Gamma^\flat,A^\flat_{0,\ell(\Gbar)}}\pa{\overline\sigma^\flat_{n,m}}}\\[1.2em]
    \bra{}^\flat_{n,n} = \sub{x_n:\Obj}
    &
      \bra{\overline\sigma;\sub{}}^\flat_{n,m} = \sub{\overline\sigma^\flat_{n,i},x_{m}} 
    \\
    & \bra{\overline\sigma;\sub{\tau,t}}^\flat_{n,m} = \sub{\bra{\overline\sigma;\tau}^\flat_{n,m},t^\flat_{j,m}} \\
  \end{array}
\]
Where in the last case, $i$ is the minimal index such that no variable
in $\sbar$ is contained in a ps-context in position after $i$ in
$\Gbar$, and $j$ is the maximal index such that no variable of $t$ is
contained in a ps-context in position before $j-1$ in $\Gbar$.
\begin{prop}
  \label{prop:ps-str-flatten-wd}
  The flattening sends derivable judgments in $\MCaTT$ onto derivable
  judgments in $\CaTT$, more precisely, chose $n$ the maximal integer
  such that no variable in $\Var{A}$ (\resp $\Var t$, $\Var \sigma$)
  appears in a context in position before $(n-1)$ in the list $\Gbar$,
  and similarly, chose $m$ the minimal integer such that no variable
  in $\Var{A}$ (\resp $\Var t$, $\Var \sigma$) appears in a context in
  position after $m$ before.
  \begin{itemize}
  \item If $\overline\Gamma\vdash A$ then
    $\overline\Gamma^\flat\vdash A^\flat_{n,m}$, (if $A = \Obj$, for
    all $i<j\leq\ell(\Gbar)$, we have
    $\Gbar^\flat\vdash \Obj^\flat_{i,j}$)
  \item If $\overline\Gamma\vdash t :A$ then
    $\overline\Gamma^\flat\vdash t^\flat_{n,m}:A^\flat_{n,m}$
  \item If $\Gbar\vdasheq A$ then
    $\Gbar^\flat\vdasheq A^\flat_{0,\ell(\Gbar)}$
  \item If $\Gbar\vdashop A$ then
    $\Gbar^\flat\vdashop A^\flat_{0,\ell(\Gbar)}$
  \item If $\overline\Gamma\vdash \overline\sigma : \overline\Delta$
    then
    $\overline\Gamma^\flat \vdash
    \overline\sigma^\flat_{n,m}:\overline\Delta^\flat$ (if $\sbar$ is
    of the form $\bra{\sbar,\sub{}}$, then there is no condition on
    $m$)
  \end{itemize}
\end{prop}
\begin{proof}
  This proof is done on mutual induction on the strucutres that we
  study
  \begin{itemize}
  \item Given a type $A$:
    \begin{itemize}
    \item If $A$ is the type $\Obj$, and for any indices
      $i<j<\ell(\Gbar)$, the associations $x_i:\Obj$ and $x_j:\Obj$
      appear in $\Gbar^\flat$. Since by
      proposition~\ref{prop:ps-flatten-wd}, $\Gbar^\flat\vdashps$,
      this shows that $\Gbar\vdash x_i:\Obj$ and
      $\Gbar\vdash x_j:\Obj$, hence $\Gbar\vdash \Hom{}{x_i}{x_j}$.
    \item If $A$ is of the form $\Hom Atu$, then the indices $n,m$
      necessarily satisfy the conditions for applying induction for
      the type $A$, and for the terms $u$ and $v$, thus by induction,
      we have that $\Gbar^\flat\vdash A^\flat_{n,m}$,
      $\Gbar^\flat\vdash t^\flat_{n,m}:A^\flat_{n,m}$ and
      $\Gbar^\flat\vdash u^\flat_{n,m}:A^\flat_{n,m}$, so this proves
      that
      \[
        \Gbar^\flat\vdash
        \Hom{A^\flat_{n,m}}{t^\flat_{n,m}}{u^\flat_{n,m}}
      \]
    \end{itemize}
  \item Given a term $\Gbar\vdash t:A$ :
    \begin{itemize}
    \item Either $t = y$ is a variable, and in this case, $A$ contains
      only variables, thus $A^\flat_{n,m} = \Susp[n,m]A$. Moreover, if
      the pairing $y:A$ appears in the ps-contexts in position $k$ in
      $\Gbar$, then $n=k, m=k+1$ and the pairing $y:\Susp[k,k+1]A$
      appears in $\Gbar^\flat$. Since by
      proposition~\ref{prop:ps-flatten-wd}, $\Gbar^\flat\vdashps$, it
      follows that
      \[
        \Gbar^\flat\vdash y:A^\flat_{k,k+1}
      \]
    \item Or $t$ is of the form $\coh_{\Dbar,B}(\sbar)$. In this case,
      by induction $\Gbar^\flat \vdash \sbar_{n,m} : \Dbar$, and
      moreover, either $\Dbar\vdashop B$, in which case we have
      $\Dbar^\flat\vdashop B^\flat_{0,\ell(\Dbar)}$, or
      $\Dbar\vdasheq B$, in which case we have
      $\Dbar^\flat\vdasheq B^\flat_{0,\ell(\Dbar)}$. In both cases,
      this shows that
      \[
        \Gbar^\flat\vdash
        \coh_{\Dbar^\flat,B^\flat_{0,\ell(\Dbar)}}(\sbar^\flat_{n,m})
        : B^\flat_{0,\ell(\Dbar)}[\sbar^\flat_{n,m}]
      \]
      Moreover, by lemma~\ref{lemma:equ-flat}
      $B^\flat_{0,\ell(\Dbar)}[\sbar^\flat_{n,m}] =
      \pa{B[\sbar]}^\flat_{n,m}$. This proves that
      \[
        \Gbar^\flat\vdash
        \coh_{\Dbar^\flat,B^\flat_{0,\ell(\Dbar)}}(\sbar^\flat_{n,m})
        : A^\flat_{n,m}
      \]
    \end{itemize}
  \item For a derivable judgment of the form $\Gbar\vdasheq A$,
    necessarily, we have that $\Gbar\vdash A$ and
    $\Var\Gamma = \Var A$, hence by induction
    $\Gbar^\flat\vdash A^\flat_{0,\ell(\Gbar)}$. Moreover, by
    lemma~\ref{lemma:equ-flat}
    \[
      \Var{\Gbar^\flat} = \Var{A^\flat}
    \]
    This proves the derivability of the following judgment
    \[
      \Gbar^\flat \vdasheq A^\flat_{0,\ell(\Gbar)}
    \]
  \item For a derivable judgment of the form $\Gbar\vdashop A$, if
    $\Gbar$ is not of dimension $0$, we necessarily have
    $A = \Hom Btu$, with $\Gbar\vdashps$, $\src\Gbar\vdash t:B$ and
    $\Var{\src\Gbar} = \Var{t:B}$. By induction, and by the variable
    conditions, we have that
    $\src\Gbar^\flat \vdash t^\flat_{0,\ell(\src{\Gbar})} :
    A^\flat_{0,\ell(\src{\Gbar})}$. Moreover, by the
    lemma~\ref{lemma:equ-flat}, $\src\Gbar^\flat = \src{\Gbar^\flat}$,
    moreover by lemma~\ref{lemma:length-src-target},
    $\ell(\src{\Gbar}) = \ell(\Gbar)$, thus
    $\src{\Gbar^\flat}\vdash t^\flat_{0,\ell(\Gbar)} :
    A^\flat_{0,\ell(\Gbar)}$, finally, again by
    lemma~\ref{lemma:equ-flat}
    \[
      \Var{\src{\Gbar}^\flat} =
      \Var{t^\flat_{0,\ell(\Gbar)}:\Var{A^\flat_{0,\ell(\Gbar)}}}
    \] The same argument holds for the judgments regarding the target,
    thus
    \[
      \Gbar^\flat\vdashop t^\flat_{0,\ell(\Gbar)} :
      A^\flat_{0,\ell(\Gbar)}
    \]
    In the case where $\Gbar$ is of dimension $0$, then it is of the
    form
    \[
      \Gbar = \bra{(f_1:\Obj);\cdots; (f_k:\Obj)}
    \]
    So $\Gbar^\flat$ can be computed explicitly as
    \[
      \Gbar^\flat = (x_0:\Obj,x_1:\Obj,f_1:\Hom{}{x_0}{x_1},
      x_2:\Obj,\cdots,x_k:\Obj,f_k:\Hom{}{x_{k-1}}{x_k})
    \]
    And we have $\Obj^\flat_{0,k} = \Hom{}{x_0}{x_k}$, so we can check
    explicitly that
    \[
      \Gbar^\flat\vdashop \Obj^\flat_{0,k}
    \]
  \item If $\Gbar\vdash \sbar : \Dbar$ is a substitution, then there
    are three cases to solve.
    \begin{itemize}
    \item If $\sbar$ is the empty substitution, for any index
      $n < \ell(\Gbar)$, we have that $\Gbar^\flat\vdash x_n:\Obj$,
      and $\bra{}^\flat_{n,n} = \sub{x_n}$ hence
      \[
        \Gbar^\flat\vdash\bra{}^\flat_{n,n} : \bra{}^\flat
      \]
    \item If $\sbar$ is of the form
      $\Gbar\vdash\bra{\sbar;\sub{}} : \bra{\Dbar;\emptycontext}$,
      then the indices $n,i$ satisfies the induction condition, and by
      induction we have that
      $\Gbar^\flat\vdash\sbar^\flat_{n,i}:\Dbar^\flat$, and
      $\Gbar^\flat\vdash x_{m} :(y:\Obj)$, hence the derivation
      \[
        \Gbar^\flat\vdash \sub{\sbar^\flat_{n,i},x_{m}} :
        \Dbar^\flat
      \]
    \item If $\sbar$ is of the form
      $\Gbar\vdash\bra{\sbar;\sub{\sigma',t}} :
      \bra{\Dbar;(\Delta',y:A)}$, then
      \[
        \bra{\sbar;\sub{\sigma',t}}^\flat_{n,m} =
        \sub{\bra{\sbar;\sigma'}^\flat_{n,m},t^\flat_{j,m}}
      \]
      all the indices satisfy the induction conditions, an by
      induction, we have the derivability of the two following
      judgments
      \begin{align*}
        \Gbar^\flat&\vdash \bra{\sbar;\tau}^\flat_{n,m} :
                     \bra{\Dbar;\Delta'}^\flat\\
        \Gbar^\flat &\vdash
                      t^\flat_{j,m}:\pa{A\bra{\sbar;\sigma'}}^\flat_{j,m}        
      \end{align*}
      Since the lemma~\ref{lemma:equ-flat} also shows,
      $\pa{A\bra{\sbar;\sigma'}}^\flat_{j,m} =
      A^\flat_{\ell(\Dbar)-1,\ell(\Dbar)}\bra{\bra{\sbar;\sigma'}^\flat_{j,m}}$,
      this proves
      \[
        \Gbar^\flat\vdash\bra{\sbar;\sub{\sigma',t}}^\flat :
        \bra{\Dbar;(\Delta',y:A)}^\flat\qedhere
      \]
    \end{itemize}
  \end{itemize}
\end{proof}

\noindent
From now on, for the sake of readability, and since they usually can
be inferred, we will often omit the indices while working with the
flattening.  Along the proof of previous proposition, we have used the
following properties, which should be proved during the induction, and
are simple enough to be left to the reader:
\begin{lemma}
  \label{lemma:equ-flat}
  The flattening is compatible with substitution application, source
  and target in dimension non $0$, and respect the equality of set of
  variables.
  \begin{enumerate}
  \item If $A$ is a type and $\sigma$ is a substitution, then
    $\pa{A[\sigma]}^\flat = A^\flat[\sigma^\flat]$
  \item If $\Gbar$ is a ps-context of dimension non $0$, then
    $\pa{\src\Gbar}^\flat = \src{\Gbar^\flat}$ and
    $\pa{\tgt\Gbar}^\flat = \tgt{\Gbar^\flat}$
  \item If $\Var\Gbar = \Var A$ then
    $\Var{\Gbar^\flat} = \Var{A^\flat}$, if $\Var{\Gbar} = \Var{t:A}$,
    then $\Var{\Gbar^\flat} = \Var{t^\flat : A^\flat}$
  \end{enumerate}
\end{lemma}

\begin{notations}
  In order to simplify the notation, we consider that the translation
  $\_^\flat$ acts directly on the judgment of the theory, and we write
  \begin{align*}
    \pa{\overline\Gamma\vdashps}^\flat &= \overline{\Gamma}^\flat\vdashps \\
    \pa{\overline\Gamma \vdash A}^\flat &= \overline\Gamma^\flat \vdash A^\flat\\
    \pa{\overline\Gamma \vdash t:A}^\flat &= \overline\Gamma^\flat \vdash t^\flat : A^\flat \\
    \pa{\overline\Gamma \vdash \overline\sigma:\overline{\Delta}}^\flat &= \overline\Gamma^\flat \vdash \overline\sigma^\flat:\overline\Delta^\flat
  \end{align*}
  where the indices that have been left implicit are the ones used in
  the proposition~\ref{prop:ps-str-flatten-wd}. We refer to these four judgments as
  \emph{monoidal ps-judgments}.
\end{notations}

\paragraph{Folding.}
Similarly, the folding operation that we have defined on ps-context
extends to types and terms in ps-contexts, along with substitutions
between ps-contexts. In order to treat the case for substitution, we
need the following notation.
% Similarly to what we have just done with the flattening, we extend
% the folding operation so that it takes into account the terms, types
% and substitutions of ps-contexts. In order to define this operation
% properly, we also need a new notation for extending lists of
% substitutions.
\[
  \sub{\overline{\sigma},t} \quad \text{is the list $\overline\sigma$
    with its last substitution extended with $t$}
\]
This allows to define the folding as a partial translation by mutual
induction as follows:
\begin{align*}
  \pa{\Hom \Obj tu}^\sharp &= \Obj
  &
    \pa{\Hom \Obj tu}^\sharp &= \Hom {A^\sharp} {t^\sharp} {u^\sharp} \\
  x^\sharp &= x
  &
    \coh_{\Gamma,A}[\sigma]^\sharp&=\coh_{\Gamma^\sharp,A^\sharp}[\sigma^\sharp]
  \\
  \sub{t}^\sharp &= \bra{}
  &
    \sub{\sigma,t}^\sharp &= \sigma^\sharp
           &
             \sub{\sigma,t}^\sharp &= \sub{\sigma^\sharp,t^\sharp}  
\end{align*}
Note that $\Obj^\sharp$ is not defined.

\begin{prop}
  \label{prop:ps-str-fold-wd}
  The folding operation sends derivable judgments in $\CaTT$ onto
  derivable judgments in $\MCaTT$, more precisely,
  \begin{itemize}
  \item If $\Gamma\vdash A$ and $A$ is not the type $\Obj$ then
    $\Gamma^\sharp\vdash A^\sharp$
  \item If $\Gamma\vdash t:A$ then
    $\Gamma^\sharp\vdash t^\sharp:A^\sharp$
  \item If $\Gamma\vdasheq A$ then $\Gamma^\sharp\vdasheq A^\sharp$
  \item If $\Gamma\vdashop A$ then $\Gamma^\sharp\vdashop A^\sharp$
  \item If $\Gamma\vdash \sigma : \Delta$ then
    $\Gamma^\sharp \vdash \sigma^\sharp:\Delta^\sharp$
  \end{itemize}
\end{prop}
\begin{proof}
  Again, this is proved by mutual induction on the structure. The case
  for substitution being very involved because of a double layered
  dependancy, we just give a sketch of the proof.
  \begin{itemize}
  \item For a type $\Gamma\vdash A$, with $A$ distinct from $\Obj$ :
    \begin{itemize}
    \item If $A$ is of the form $\Hom\Obj tu$, then $A^\sharp = \Obj$,
      and by proposition~\ref{prop:ps-fold-wd}, we have that
      $\Gamma^\sharp\vdashps$, hence $\Gamma^\sharp\vdash \Obj$.
    \item If $A$ is on the form $\Hom Btu$, with $B\neq\Obj$, then
      necessarily we have $\Gamma\vdash B$, $\Gamma\vdash t:B$ and
      $\Gamma\vdash u:B$, and thus by induction cases on types and
      terms, we have $\Gamma^\sharp\vdash B^\sharp$,
      $\Gamma^\sharp\vdash t^\sharp:B^\sharp$ and
      $\Gamma^\sharp\vdash u^\sharp:B^\sharp$. This proves
      $\Gamma^\sharp\vdash A^\sharp$.
    \end{itemize}
  \item For a term $\Gamma\vdash t:A$, with $A\neq\Obj$:
    \begin{itemize}
    \item If $t = x$ is a variable, then since $\Gamma$ is a
      ps-context, necessarily $A$ contains only variables, and the
      pairing $x:A$ appears in $\Gamma$. By definition, the pairing
      $x:A^-$ appears in $\Gamma^\sharp$, and thus
      $\Gamma^\sharp\vdash x:A^-$. Since $A$ contains only variables,
      we have that $A^- = A^\sharp$, and thus
      $\Gamma^\sharp\vdash A^\sharp$.
    \item If $t = \coh_{\Delta,B}(\sigma)$ is a coherence, then
      $t^\sharp = \coh_{\Delta^\sharp,B^\sharp}(\sigma^\sharp)$. We
      necessarily have $\Gamma\vdash\sigma:\Delta$, and by induction,
      $\Gamma^\sharp\vdash\sigma^\sharp:\Delta^\sharp$. Moreover,
      either $\Delta\vdasheq B$, in which case the induction gives
      $\Delta^\sharp\vdasheq B^\sharp$, or $\Delta\vdashop B$, in
      which case induction gives $\Delta^\sharp\vdasheq B^\sharp$. In
      both cases, this proves that
      $\Gamma^\sharp\vdash t^\sharp : B^\sharp[\sigma^\sharp]$, and
      since by lemma~\ref{lemma:equ-fold},
      $B^\sharp[\sigma^\sharp] = \pa{B[\sigma]}^\sharp$, this proves
      $\Gamma^\sharp\vdash t^\sharp:A^\sharp$.
    \end{itemize}
  \item For a judgment of the form $\Gamma\vdasheq A$, we have
    $\Gamma\vdash A$ and $\Var\Gamma = \Var A$, so by induction, we
    also have $\Gamma^\sharp\vdash A^\sharp$. Moreover, we have by
    lemma~\ref{lemma:equ-fold},
    $ \Var{\Gamma^\sharp}= \Var{A^\sharp} $ and thus
    $\Gamma^\sharp\vdasheq A^\sharp$.
  \item For a judgment of the form $\Gamma\vdashop A$, necessarily we
    have $A = \Hom Btu$, with $\src\Gamma\vdash t:B$ and
    $\tgt\Gamma\vdash u:B$, and $\Var{\src\Gamma} = \Var{t:B}$,
    $\Var{\tgt\Gamma} = \Var{u:B}$.
    \begin{itemize}
    \item If $B$ is the type $\Obj$, then $A^\sharp = \Obj$ and $t$
      and $u$ are necessarily variables. The variable conditions then
      imply that $\src\Gamma$ and $\tgt\Gamma$ are just one
      point. This is only possible when $\Gamma$ is of dimension $1$,
      \ie $\Gamma^\sharp$ is a list of containing all contexts
      isomorphic to $\D^0$, which proves that
      $\Gamma^\sharp\vdashop \Obj$.
    \item If $B$ is not the type $\Obj$, then
      $A^\sharp = \Hom {B^\sharp}{t^\sharp}{u^\sharp}$. By induction
      we have $\pa{\src{\Gamma}}^\sharp\vdash t^\sharp:A^\sharp$,
      with, by lemma~\ref{lemma:equ-fold},
      $\Var{{\src\Gamma}^\sharp} = \Var{t^\sharp:A^\sharp}$. Again by
      lemma~\ref{lemma:equ-fold}, we have
      $\pa{\src{\Gamma}}^\sharp = \src{\Gamma^\sharp}$, hence,
      \begin{align*}
        \src{\Gamma^\sharp} &\vdash t^\sharp : A^\sharp\\
        \Var{\src{\Gamma^\sharp}} &= \Var{t^\sharp:A^\sharp}
      \end{align*}
      The demonstration is symmetric for the case of $\tgt\Gamma$,
      hence this proves that $\Gamma^\sharp\vdashop A^\sharp$
    \end{itemize}
  \item For substitutions :
    \begin{itemize}
    \item In the case of the substitution
      $\Gamma\vdash\sub{x} : \D^0$, then $\sigma^\sharp = \bra{}$, and
      since $\Gamma^\sharp\vdash$, it follows that
      $\Gamma^\sharp\vdash \bra{} : \bra{}$
    \item For a substitution of the form
      $\Gamma\vdash \sub{\sigma,t,u} : (\Delta,y:\Obj, f:\Hom {}xy)$,
      we have
      $\sub{\sigma,t,u}^\sharp =
      \bra{\sigma^\sharp;\sub{u^\sharp}}$. Necessarily, $t$ is a
      variable in $\Gamma$, and thus this provides a split
      $\Gamma^\sharp = \Gbar_1@\Gbar_2$, with all variables in
      $\Gbar_1$ appearing before $u$ and $\Gamma$ and all variables in
      $\Gbar_2$ appearing after $u$ in $\Gamma$. By induction, we have
      $\Gamma^\sharp\vdash \sigma^\sharp : \Delta^\sharp$. Moreover
      $\sigma^\sharp$ contains only variables in $\Gbar_1$, thus in
      fact $\Gbar_1\vdash \sigma^\sharp:\Delta^\sharp$. Similarly,
      because of the way $u$ uses the variables,
      $\Gbar_2\vdash u^\sharp : \Obj$. This justifies the derivability of the
      substitution $\Gbar_2\vdash\sub{u} : (f:\Obj)$, and hence, this
      proves that
      \[
        \Gbar_1@\Gbar_2\vdash\bra{\sigma,\sub{u^\sharp}}:\bra{\Delta;(f:\Obj)}
      \]
    \item In the case of a substitution
      $\Gamma\vdash\sub{\sigma,t,u} : (\Delta,y:A,f:\Hom{}xy)$, we
      have that
      $\sub{\sigma,t,u}^\sharp =
      \sub{\sigma^\sharp,t^\sharp,u^\sharp}$. By induction,
      $\Delta^\sharp = \bra{\Dbar_1;\Delta'}$,
      $\sigma^\sharp = \bra{\sbar;\sigma'}$ and we have a split of the
      form $\Gamma^\sharp = \Gbar_1@\Gbar_2$, such that
      $\Gbar_1@\Gbar_2\vdash \sub{\sbar_1;\sigma'} :
      \bra{\Dbar_1';\Delta'}$, with $\Gbar_1\vdash\sbar_1:\Dbar_1$ and
      $\Gbar_2\vdash\sigma':\Delta'$. Moreover, by applying the
      induction twice, we have
      $\Gbar_2\vdash t^\sharp:A^\sharp[\sigma']$ and
      $\Gbar_2 \vdash u:A^\sharp[\sub{\sigma',t^\sharp}]$, thus
      $\Gbar_2\vdash\sub{\sigma',t^\sharp,u^\sharp} :
      (\Delta,y:A^\sharp,f:\Hom{} xy)$. This justifies that
      \[
        \Gbar_1@\Gbar_2
        \vdash\sub{\sbar_1;\sub{\sigma',t^\sharp,u^\sharp}} :
        \bra{\Dbar_1;(\Delta'; y:A^\sharp;f : \Hom{}xy)}
      \]
    \end{itemize}
  \end{itemize}
\end{proof}
\noindent
Similarly to the case of the flattening, we have used the following
properties, which should be proved during the induction, but are
simple enough to be left out
\begin{lemma}
  \label{lemma:equ-fold}
  The folding operation respects application of substitutions, source
  and target of ps-contexts and preserves equality of variables
  \begin{enumerate}
  \item If $A$ is a type distinct from $\Obj$ and $\sigma$ is a
    substitution, $\pa{A[\sigma]}^\sharp = A^\sharp[\sigma^\sharp]$
  \item If $\Gamma$ is a ps-context,
    $\pa{\src\Gamma}^\sharp = \src{\Gamma^\sharp}$ and
    $\pa{\tgt\Gamma}^\sharp = \tgt{\Gamma^\sharp}$
  \item If $\Var\Gamma = \Var A$, then
    $\Var{\Gamma^\sharp} = \Var{A^\sharp}$, and if
    $\Var\Gamma = \Var{t:A}$, then
    $\Var{\Gamma^\sharp} = \Var{t^\sharp:A^\sharp}$
  \end{enumerate}
\end{lemma}

\begin{notations}
  Similarly, we consider $\_^\sharp$ as acting on judgments on the
  theory and denote
  \begin{align*}
    \pa{\Gamma\vdashps}^\sharp &= \Gamma^\sharp\vdashps \\
    \pa{\Gamma \vdash A}^\sharp &= \Gamma^\sharp \vdash A^\sharp\\
    \pa{\Gamma \vdash t:A}^\sharp &= \Gamma^\sharp \vdash t^\sharp: A^\sharp\\
    \pa{\Gamma \vdash \sigma:\Delta}^\sharp &= \Gamma^\sharp \vdash\sigma^\sharp:\Delta^\sharp
  \end{align*}
  These four judgments be called \emph{ps-judgments} in the theory
  $\CaTT$. In this case they are no different from usual judgments
  between ps-contexts, but they play an important role in their
  interaction with the theory $\MCaTT$.
\end{notations}

\paragraph{Interaction between flattening and folding.}
In proposition~\ref{prop:ps-flatten-fold}, we have proved that the
flattening and the folding were inverse of each other on ps-contexts,
we now show that this extends to all ps-judgments, \ie these
operations are inverse on terms, types and substitutions in
ps-contexts.
\begin{prop}
  \label{prop:flatten-fold}
  For any monoidal ps-judgment $J$ in $\MCaTT$,
  \[
    (J^\flat)^\sharp = J
  \]
  For any ps-judgment $J$ in $\CaTT$,
  \[
    (J^\sharp)^\flat \simeq J \qquad \text{up to renaming of the
      variables of type $\Obj$.}
  \]
\end{prop}

\begin{proof}
  Note that we have already proved the equality in the case of a
  judgment of the form $\Gamma\vdashps$. The other cases are done by
  mutual induction on the structure.
  \begin{itemize}
  \item For types:
    \begin{itemize}
    \item In the case of the type $\Obj$, we have that
      \[
        \pa{\pa{\Obj}^\flat_{n,m}}^\sharp =
        \pa{\Hom\Obj{x_n}{x_m}}^\sharp = \Obj
      \]
    \item In the case of the type $\Hom Atu$, we have
      \[
        \pa{\pa{\overline\Gamma\vdash \Hom Atu}^\flat}^\sharp =
        \Hom{(A^\flat)^\sharp}{(t^\flat)^\sharp}{(u^\flat)^\sharp}
      \]
      and by induction $\pa{A^\flat}^\sharp = A$,
      $\pa{t^\flat}^\sharp = t$ and $\pa{u^\flat}^\sharp = u$, which
      proves that
      \[
        \pa{\pa{\Hom Atu}^\flat}^\sharp = \Hom Atu
      \]
    \end{itemize}
  \item For terms :
    \begin{itemize}
    \item In the case of a variable, we have
      \[
        \pa{x^\flat}^\sharp = x^\sharp = x
      \]
    \item In the case of a coherence, we have
      \[
        \pa{\pa{\coh_{\Gbar,A}(\sbar)}^\flat}^\sharp =
        \pa{\coh_{\Gbar^\flat,A^\flat}(\sbar^\flat)}^\sharp =
        \coh_{\pa{\Gbar^\flat}^\sharp,\pa{A^\flat}^\sharp}\pa{\pa{\sbar^\flat}^\sharp}
      \]
      By induction, $\pa{\Gbar^\flat}^\sharp = \Gbar$,
      $\pa{A^\flat}^\sharp = A$ and $\pa{\sbar^\flat}^\sharp = \sbar$,
      hence
      \[
        \pa{\pa{\coh_{\Gbar,A}(\sbar)}^\flat}^\sharp =
        \coh_{\Gbar,A}(\sbar)
      \]
    \end{itemize}

  \item For substitutions :
    \begin{itemize}
    \item In the case of the empty list, we have
      \[
        \pa{\bra{}^\flat_{n,m}}^\sharp = \sub{x_n}^\sharp = \bra{}
      \]
    \item In the case of a non empty list, notice that the none of the
      component of the list can be empty since this is not allowed for
      substitutions in monoidal ps-contexts. In the case where the
      last substitution of the list is of lentgh $1$, we have
      \[
        \pa{\bra{\sbar;\sub{t}}^\flat}^\sharp =
        \sub{\sbar^\flat,x_{k+1},t^\flat}^\sharp =
        \bra{\pa{\sbar^\flat}^\sharp,\sub{\pa{t^\flat}^\sharp}}
      \]
      since $x_{k+1}$ is necessarily of dimension $0$. The induction
      gives the equalities $\pa{\sbar^\flat}^\sharp = \sbar$ and
      $\pa{t^\flat}^\sharp = t$, which proves that
      \[
        \pa{\bra{\sbar;\sub{t}}^\flat}^\sharp = \bra{\sbar;\sub{t}}
      \]
    \item In the case of a non emtpy list, with the last substitution
      of length $n>1$, we have
      \[
        \pa{\bra{\sbar;\sub{\tau,t}}^\flat}^\sharp =
        \sub{\bra{\sbar;\tau}^\flat,t^\flat}^\sharp =
        \sub{\pa{\bra{\sbar;\tau}^\flat}^\sharp,\pa{t^\flat}^\sharp}
      \]
      The induction provides the equalities
      $\pa{\bra{\sbar;\tau}^\flat}^\sharp = \bra{\sbar;\tau}$ and
      $\pa{t^\flat}^\sharp = t$, hence we have
      \[
        \pa{\bra{\sbar;\sub{\tau,t}}^\flat}^\sharp =
        \bra{\sbar;\sub{\tau,t}}
      \]
    \end{itemize}
  \end{itemize}
  For the converse equality, the same mutually inductive arguments
  applies, but one has to carry all the renaming of variables of
  dimension $0$ everywhere. We do not give a full proof here, since
  the equality in this direction will not be useful for us.
\end{proof}

\subsection{Translations for the syntactic categories}
We have defined two operations of flattening and folding that
establish a correspondence between the judgments in a ps-context of
$\CaTT$ and the judgments in a monoidal ps-context of $\MCaTT$. We now
extend these operations to all judgments on both type theories,
defining a pair of functors between $\Syn{\CaTT}$ and
$\Syn{\MCaTT}$. We also show that these functors respect a lot of the
structure of category with families of both syntactic categories. We
will see in the next section what is the exact structure that is
missing, and how this reflects on the models.
% The aim is now to extend the flattening and folding operations on
% ps-judgments to all judgments on our theory, in order to define
% functors between $\Syn{\CaTT}$ and $\Syn{\MCaTT}$ which respect most
% of the structure of category with families. As we will see later on,
% these do not define proper morphisms of category with families,
% since part of the structure is left out, and this defect exactly
% what gives us enough room to manoeuvre and highlight the link
% between categories and monoidal categories as type theories.
\paragraph{Flattening.}
We extend the falttening operation to all judgments of the type
theory, defining a translation that we call $\tr$ which associates to
any judgment in $\MCaTT$ a judgment in $\CaTT$. This is done by
induction on the structure of the type theory.
\begin{align*}
  \tr\emptycontext &= (x_0 : \Obj)
  &
    \tr{(\Gamma, y : A)} &= (\tr\Gamma, y:\tr A)
  \\
  \tr\Obj &= \Hom{\Obj}{x_0}{x_0}
  &
    \tr{\Hom Axy} &= \Hom{\tr A}{\tr x}{\tr y}
  \\
  \tr x &= x
  &
    \tr\pa{\coh_{\overline\Gamma,A}(\overline\sigma)} &= \pa{\coh_{\overline\Gamma, A}}^\flat(\tr{\overline\sigma})
  \\
  \tr\sub{} &= \sub{x_0}
  &
    \tr{\sub{\sigma,t}} &= \sub{\tr\sigma, \tr t}
  \\
  \tr[] &= \sub{x_0}
  &
    \tr\bra{\overline\sigma;\tau} &= \sub{\tr\overline\sigma, \tr\tau}                         
\end{align*}

\begin{prop}
  \label{prop:almost-cwf-mor}
  This translation sends derivable judgments in $\MCaTT$ onto
  derivable judgments in $\CaTT$, more precisely
  \begin{itemize}
  \item If $\Gamma \vdash$ then $\tr\Gamma\vdash$
  \item If $\Gamma\vdash A$ then $\tr\Gamma\vdash \tr A$ and
    $\tr(\Gamma,y:A) = (\tr\Gamma,y:\tr A)$
  \item If $\Gamma\vdash t:A$ then $\tr\Gamma\vdash \tr t :\tr A$
  \item If $\Gamma\vdash \sigma : \Delta$ then
    $\tr \Gamma\vdash \tr \sigma : \tr\Delta$ and
    $\tr\sub{\sigma,t} = \sub{\tr\sigma,\tr t}$
  \item If $\Gamma \vdash \overline\sigma : \overline\Delta$ then
    $\tr\Gamma\vdash \tr\overline\sigma : \overline{\Delta}^\flat$
  \end{itemize}
\end{prop}
\begin{proof}
  All these statements are proved by mutual induction on the structure
  of a type theory. In the case of substitutions to a monoidal
  ps-context, we just give a sketch of proof, since it contains two
  layers of inductions, which makes the reasoning hard to track if we
  write it all completely.
  \begin{itemize}
  \item A context is either the empty context $\emptycontext$ or of
    the form $(\Gamma,y:A)$.
    \begin{itemize}
    \item In the case of the empty context, we have that
      $\tr\emptycontext = (x_0:\Obj)$, and thus
      $\tr\emptycontext \vdash$.
    \item In the case of a context of the form $(\Gamma,y:A)$, we
      necessarily have that $\Gamma\vdash A$, and thus by induction on
      the case for types, $\tr\Gamma\vdash\tr A$, which proves that
      $\tr(\Gamma,y:A)\vdash$.
    \end{itemize}
    Note that that for any context $\Gamma$ in $\MCaTT$, we have
    $\tr\Gamma\vdash x_0:\Obj$, since it is already true for the empty
    context.
  \item A type is either $\Obj$ or of the form $\Hom Atu$.
    \begin{itemize}
    \item In the case of the type $\Gamma\vdash \Obj$, we have
      $\tr\Obj = \Hom \Obj {x_0}{x_0}$, and since we always have
      $\tr\Gamma\vdash x_0:\Obj$, this proves that
      $\tr\Gamma\vdash\tr\Obj$.
    \item In the case of a type of the form $\Gamma\vdash \Hom Atu$,
      we necessarily have $\Gamma\vdash t:A$ and $\Gamma\vdash
      u:A$. The induction case for the term on both judgments shows
      that $\tr\Gamma\vdash \tr u: \tr A$ and
      $\tr\Gamma\vdash \tr t : \tr A$. This proves
      $\tr\Gamma\vdash \tr\pa{\Hom Atu}$
    \end{itemize}
  \item A term $\Gamma\vdash t:A$ is either a variable or a coherence.
    \begin{itemize}
    \item For a variable $\Gamma\vdash x:A$, we then have that the
      pairing $x:A$ appears in the list $\Gamma$, and thus by
      construction, the pairing $x:\tr A$ appears in the list
      $\tr\Gamma$. This proves that $\tr\Gamma\vdash x : \tr A$.
    \item For a coherence of the form $t = \coh_{\Dbar,B}(\sbar)$, we
      have
      \[
        \tr t = \pa{\coh_{\Dbar,B}(\id{\Dbar})}^\flat[\sbar]
      \]
      By the induction case for substitution towards a monoidal
      ps-context, we have $\tr\Gamma\vdash\tr\sigma:\Dbar^\flat$, and
      by the proposition~\ref{prop:ps-str-flatten-wd}, we have that
      $\Dbar^\flat\vdash\pa{\coh_{\Dbar,B}(\id{\Dbar})}^\flat$, so
      this proves $ \tr\Gamma\vdash\tr t : B^\flat[\tr\sbar] $, and
      since, by lemma~\ref{lemma:equ-iota},
      $B^\flat[\tr\sbar] = \tr\pa{B[\sbar]}$, this shows that
      $ \tr\Gamma\vdash\tr t : \tr A $.
    \end{itemize}
  \item A substitution is either $\sub{}$ or of the form
    $\sub{\sigma,t}$.
    \begin{itemize}
    \item For the substitution $\Gamma\vdash \sub{}:\emptycontext$, we
      have $\iota\sub{} = \sub{x_0}$, and since we necessarily have
      that $\tr\Gamma\vdash x_0:\Obj$, this proves
      $\tr\Gamma\vdash\sub{x_0:\Obj}:(x_0:\Obj)$.
    \item For a substitution of the form
      $\Gamma\vdash\sub{\sigma,t}:(\Delta,y:A)$, we have
      $\tr\sub{\sigma,t} = \sub{\tr\sigma,\tr t}$, and by induction
      cases on substitutions on types and on terms, we have
      $\tr\Gamma\vdash\tr\sigma:\tr\Delta$, $\tr\Delta\vdash\tr A$ and
      $\tr\Gamma\vdash\tr t : \tr\pa{A[\sigma]}$. Since, by
      lemma~\ref{lemma:equ-iota},
      $\tr\pa{A[\sigma]} = \tr A[\tr \sigma]$, this proves that the
      substitution
      $\tr{\Gamma}\vdash\sub{\tr\sigma,\tr t} : (\tr\Delta,y:\tr A)$
      is derivable.
    \end{itemize}
  \item A substitution to a monoidal ps-context is either $\bra{}$ or
    of the form $\bra{\sbar,\tau}$.
    \begin{itemize}
    \item For the substitution $\Gamma\vdash\bra{}:\bra{}$, we have
      $\tr\bra{} = \sub{x_0}$ and since we always have
      $\tr\Gamma\vdash x_0:\Obj$, this proves that
      $\tr\Gamma\vdash\sub{x_0}:(x_0:\Obj)$.
    \item For a substitution of the form
      $\Gamma\vdash\bra{\sbar;\sub{}}:\bra{\Dbar;\bra{}}$, we have
      that $\tr\bra{\sbar;\bra{}} = \bra{\tr\sbar;\sub{x_0}}$, and by
      the induction, we have $\Gamma\vdash\sbar:\Dbar$ and
      $\tr\Gamma\vdash x_0:\Obj$. This proves that
      $\tr\Gamma\vdash \sub{\tr\sigma,x_0} :
      \bra{\Dbar,\bra{}}^\flat$.
    \item For a substitution of the form
      \[
        \Gamma\vdash\sub{\tau,t,u}:\Delta',z:B,f:\Hom{}yz
      \] then by induction we have that
      $\tr\Gamma\vdash \iota\bra{\sbar;\tau}
      :\bra{\Dbar,\Delta'}^\flat$, and by two successive induction
      $\tr\Gamma\vdash \tr t:\tr\pa{B[\sbar;\tau]}$ and
      $\tr\Gamma\vdash \tr
      u:\tr\pa{\pa{\Hom{}yz}[\sbar;\sub{\tau,t}]}$. Using the
      lemma~\ref{lemma:equ-iota} twice, we get the derivation of the
      judgment $\tr\Gamma\vdash\tr\sub{\sigma,t,u}:\tr A$
    \end{itemize}
  \end{itemize}
\end{proof}
\begin{note}
  \label{note:obstruction-terminal}
  This proposition may seem to indicate that $\tr$ defines a morphism
  of categories with families, but crucially this is not actually the
  case. In fact $\tr$ preserves all the structural rules of the type
  theory but one: it does not send the terminal object onto the
  terminal object. Indeed, the terminal object in $\Syn{\MCaTT}$ is
  the context empty context $\emptycontext$, and it is sent onto the
  context $(x_0:\Obj)$ in $\Syn{\CaTT}$, which is not terminal.
\end{note}

\noindent
Along the proof of the proposition~\ref{prop:almost-cwf-mor}, we have
used some properties of the translation $\iota$, which should be
proved by induction together with the statements, but which we have
left out.
\begin{lemma}
  \label{lemma:equ-iota}
  The translation $\iota$ respects the two types of substitutions.
  \begin{enumerate}
  \item If $A$ is a type and $\sbar$ is a substitution to a monoidal
    ps-context, then $\iota\pa{A[\sbar]} = A^\flat [\iota \sbar]$
  \item If $A$ is a type and $\sigma$ is a substitution, then
    $\iota\pa{A[\sigma]} = \iota A [\iota\sigma]$
  \end{enumerate}
\end{lemma}



\paragraph{Folding.}
Similarly, we extend the folding operation defined on judgments in a
ps-context to any judgment, by a translation $\kappa$ which sends
judgments of $\CaTT$ onto judgments of $\MCaTT$.
\begin{align*}
  \kappa\emptycontext &= \emptycontext
  &
    \kappa(\Gamma,x:A) &=\left\{
                         \begin{array}{l@{\quad}l}
                           \kappa\Gamma & \text{if $A = \Obj$}\\
                           (\kappa\Gamma,x:\kappa A) & \text{otherwise}
                         \end{array}\right.\\
  \kappa\pa{\Hom\Obj tu} &= \Obj
  &
    \kappa\pa{\Hom Atu} &= \Hom{\kappa A}{\kappa t}{\kappa u}\\
  \kappa x &= x
  &
    \kappa\pa{\coh_{\Gamma,A}(\sigma)} &= \pa{\coh_{\Gamma,A}}^\sharp(\kappa^\sharp\sigma)\\
  \kappa\sub{} &= \sub{}
  &
    \kappa\sub{\sigma,t} &= \left\{
                           \begin{array}{l@{\quad}l}
                             \kappa\sigma & \text{if $\dim t = 0$}\\
                             \sub{\kappa\sigma,\kappa t} &\text{otherwise}
                           \end{array}
                                                           \right.\\
  \kappa^\sharp\sub{t} &= \bra{}
  &
    \kappa^\sharp\sub{\sigma,t} &=\left\{
                                  \begin{array}{l@{\quad}l}
                                    \bra{\kappa^\sharp\sigma;\sub{}} & \text{if $\dim t = 0$} \\
                                    \sub{\kappa^\sharp\sigma,\kappa t}&\text{otherwise}
                                  \end{array}
                                                                        \right.
\end{align*}
Note that again, the translation $\kappa$ is not properly defined on
the type $\Obj$
\begin{prop}
  \label{prop:retract-almost-cwf-mor}
  This translation sends derivable judgments in $\CaTT$ onto
  derivable judgments in $\MCaTT$, more precisely
  \begin{itemize}
  \item If $\Gamma \vdash$ then $\kappa\Gamma\vdash$
  \item If $\Gamma\vdash A$ with $A\neq\Obj$, then
    $\kappa\Gamma\vdash \kappa A$ and
    $\kappa(\Gamma,y:A) = (\tr\Gamma,y:\kappa A)$
  \item If $\Gamma\vdash t:A$ with $A\neq\Obj$, then
    $\kappa\Gamma\vdash \kappa t :\kappa A$
  \item If $\Gamma\vdash \sigma : \Delta$ then
    $\kappa \Gamma\vdash \kappa \sigma : \kappa\Delta$ and when
    $\dim t > 1$, $\kappa\sub{\sigma,t} = \sub{\kappa\sigma,\kappa t}$
  \item If $\Gamma \vdash \sigma : \Delta$ then
    $\kappa\Gamma\vdash \kappa^\sharp\sigma : {\Delta}^\sharp$
  \end{itemize}
\end{prop}
\begin{proof}
  All these statements are proved by mutual induction on the structure
  that we study
  \begin{itemize}
  \item A context is either $\emptycontext$ or of the form
    $(\Gamma,y:A)$.
    \begin{itemize}
    \item In the case of $\emptycontext$, we have that
      $\kappa\emptycontext = \emptycontext$ and thus
      $\kappa\emptycontext\vdash$.
    \item For a context of the form $(\Gamma,y:\Obj)$, we have that
      $\kappa(\Gamma,y:\Obj) = \kappa\Gamma$, and thus by induction
      $\kappa(\Gamma,y:\Obj)\vdash$. 
    \item For a context of the form
      $(\Gamma,y:A)$, with $A\neq\Obj$, we have that
      $\kappa(\Gamma,y:A) = (\kappa\Gamma,y:\kappa A)$. By induction,
      we have $\kappa\Gamma\vdash$ and $\kappa\Gamma\vdash \kappa A$, thus
      this proves $\kappa(\Gamma,y:A)\vdash$
    \end{itemize}
  \item A term distinct from $\Obj$ is necessarily of the form
    $\Gamma\vdash\Hom Atu$.
    \begin{itemize}
    \item If $A = \Obj$, then we have $\kappa\pa{\Hom\Obj tu} =
      \Obj$. By induction we have that $\kappa\Gamma\vdash$, and thus
      $\kappa\Gamma\vdash\Obj$.
    \item If $A$ is not the type $\Obj$, we have
      $\kappa\pa{\Hom Atu} = \Hom{\kappa A}{\kappa t}{\kappa
        u}$. Moreover, necessarily we have $\Gamma\vdash t:A$ and
      $\Gamma\vdash u:A$, thus by induction we also have,
      $\kappa\Gamma\vdash \kappa t: \kappa A$ and
      $\kappa\Gamma\vdash\kappa u: \kappa A$. This proves that
      $\kappa\Gamma\vdash\kappa\pa{\Hom Atu}$
    \end{itemize}
  \item A term $\Gamma\vdash t:A$ is either a variable or a coherence.
    \begin{itemize}
    \item For a variable $y$ of type $A$ which is not $\Obj$, the
      pairing $y:A$ is contained in the context $\Gamma$, thus the
      pairing $(y:\kappa A)$ is contained in the context
      $\kappa\Gamma$, hence we have $\kappa\Gamma\vdash y:\kappa A$.
    \item In the case of a coherence $t = \coh_{\Delta,B}(\sigma)$, we
      have that
      \[
        \kappa\pa{\coh_{\Delta,B}(\sigma)} =
        \pa{\coh_{\Delta,B}}^\sharp(\kappa^\sharp\sigma)
      \]
      By the proposition~\ref{prop:ps-str-fold-wd}, we have that
      $\Delta^\sharp\vdash \pa{\coh_{\Delta,B}}(\id\Delta)$, and by
      induction we have
      $\kappa\Gamma\vdash\kappa^\sharp\sigma : \Delta^\sharp$. This
      proves that
      \[
        \kappa\Gamma\vdash
        \pa{\coh_{\Delta,B}}^\sharp(\kappa^\sharp\sigma) :
        B^\sharp[\kappa^\sharp\sigma]
      \]
      Since by lemma~\ref{lemma:equ-kappa},
      $ B^\sharp[\kappa^\sharp\sigma] = \kappa\pa{B[\sigma]}$, this
      proves that $\kappa\Gamma\vdash \kappa t : \kappa A$.
    \end{itemize}
  \item A substitution is either $\sub{}$ or it is of the form
    $\sub{\sigma,t}$.
    \begin{itemize}
    \item In the case of the substitution
      $\Gamma\vdash\sub{}:\emptycontext$, we have
      $\kappa\sub{} = \sub{}$ and
      $\kappa\emptycontext=\emptycontext$. So we have
      $\kappa\Gamma\vdash \kappa\sub{}:\kappa\emptycontext$.
    \item In the case of a substitution of the form
      $\Gamma\vdash\sub{\sigma,t}:(\Delta,y:\Obj)$, we necessarily
      have $\Gamma\vdash \sigma:\Delta$, thus by induction
      $\kappa\Gamma\vdash\kappa\sigma:\kappa\Delta$. Moreover,
      necessarily $\dim t = 1$, and thus
      $\kappa\sub{\sigma,t} = \kappa\sigma$. This proves that
      $\kappa\Gamma\vdash\kappa\sub{\sigma,t}:\kappa(\Delta,y:\Obj)$.
    \item In the case of a substitution of the form
      $\Gamma\vdash\sub{\sigma,t}:(\Delta,y:A)$, with $A$ distinct
      from $\Obj$, then
      $\kappa\sub{\sigma,t} = \sub{\kappa\sigma,\kappa t}$ and we
      necessarily have that $\Gamma\vdash\sigma : \Delta$,
      $\Delta\vdash A$ and $\Gamma\vdash t:A[\sigma]$. So by
      induction, we have that
      $\kappa\Gamma\vdash\kappa\sigma:\kappa\Delta$,
      $\kappa\Delta\vdash\kappa A$ and also
      $\kappa\Gamma\vdash\kappa t : \kappa\pa{A[\sigma]}$. Since, by
      lemma~\ref{lemma:equ-kappa},
      $\kappa\pa{A[\sigma]} = \kappa A[\kappa\sigma]$, this proves
      that
      \[
        \kappa\Gamma\vdash\kappa\sub{\sigma,t} : \kappa(\Delta,y:A)
      \]
    \end{itemize}
  \item A substitution is either $\sub{}$ or it is of the form
    $\sub{\sigma,t}$.
    \begin{itemize}
    \item In the case of the substitution
      $\Gamma\vdash\sub{}:\emptycontext$, we have
      $\kappa^\sharp\sub{} = \bra{}$. So we have
      $\kappa^\sharp\Gamma\vdash \bra{}:\bra{}$.
    \item In the case of a substitution of the form
      $\Gamma\vdash\sub{\sigma,t}:(\Delta,y:\Obj)$, we necessarily
      have $\Gamma\vdash \sigma:\Delta$, thus by induction
      $\kappa\Gamma\vdash\kappa^\sharp\sigma:\Delta^\sharp$. Moreover,
      necessarily $\dim t = 1$, and thus
      $\kappa^\sharp\sub{\sigma,t} =
      \bra{\kappa^\sharp\sigma,\sub{}}$. This proves that
      $\kappa\Gamma\vdash\kappa^\sharp\sub{\sigma,t}:(\Delta,y:\Obj)^\sharp$.
    \item In the case of a substitution of the form
      $\Gamma\vdash\sub{\sigma,t}:(\Delta,y:A)$, with $A$ distinct
      from the type $\Obj$, then
      $\kappa^\sharp\sub{\sigma,t} = \sub{\kappa^\sharp\sigma,\kappa
        t}$ and we necessarily have that
      $\Gamma\vdash\sigma : \Delta$, $\Delta\vdash A$ and
      $\Gamma\vdash t:A[\sigma]$. So by induction, we have that
      $\kappa\Gamma\vdash\kappa^\sharp\sigma:\Delta^\sharp$,
      $\kappa\Delta\vdash\kappa A$ and also
      $\kappa\Gamma\vdash\kappa t : \kappa\pa{A[\sigma]}$. Since by
      the lemma~\ref{lemma:equ-kappa},
      $\kappa\pa{A[\sigma]} = \kappa A[\kappa^\sharp\sigma]$, this
      proves that
      $\kappa\Gamma\vdash\kappa^\sharp\sub{\sigma,t} :
      (\Delta,y:A)^\sharp$.
    \end{itemize}
  \end{itemize}
\end{proof}
\begin{note}
  Again this proposition states that $\kappa$ almost defines a
  morphism of categories with families from $\Syn{\CaTT}$ to
  $\Syn{\MCaTT}$. Here it fails to do so because it is partial, there
  is no image for the type $\Obj$, nor for any term of dimension $0$.
\end{note}

\noindent Again, during the proof of the
proposition~\ref{prop:retract-almost-cwf-mor}, we have used some
properties followed by $\kappa$ and $\kappa^\sharp$, which should be
proved by induction together with these statements, but that we omit
\begin{lemma}
  \label{lemma:equ-kappa}
  The translations $\kappa$ and $\kappa^\sharp$ respect the
  application of substitutions.
  \begin{enumerate}
  \item If $A$ is a type and $\sigma$ is a substitution to a
    ps-context,
    $\kappa\pa{A[\sigma]} = \kappa A[\kappa^\sharp \sigma]$
  \item If $A$ is a type and $\sigma$ is a substitution,
    $\kappa\pa{A[\sigma]} = \kappa A[\kappa \sigma]$
  \end{enumerate}
\end{lemma}



\paragraph{Interaction between flattening and folding.}
The previous result exhibiting the flattening and folding as inverses
for ps-judgments extends to the full fledged type theory only in one
direction.
\begin{prop}
  \label{prop:retract-is-retract}
  the functor $\kappa$ is a retract of the functor $\tr$
  \[
    \kappa \circ \tr \qeq \id{\Syn{\MCaTT}}
  \]
\end{prop}
\begin{proof}
  This is proven by structural induction on the various objects of the
  theory
  \begin{itemize}
  \item Context are either of the form $\emptycontext$, or of the form
    $(\Gamma,x:A)$.
    \begin{itemize}
    \item For $\emptycontext$, we have
      $\tr\emptycontext = (x_0 : \Obj)$, and
      $\kappa (x_0 : \Obj) = \emptycontext$, thus
      $\kappa(\tr \emptycontext) = \emptycontext$.
    \item For a context of the form $(\Gamma,x:A)$, we have
      $\tr(\Gamma,x:A) = (\tr\Gamma,x:\tr A)$, and
      $\kappa(\tr(\Gamma,x:A)) = (\kappa(\tr\Gamma),x:\kappa(\tr
      A))$. By the induction case for context, we have
      $\kappa(\tr \Gamma) = \Gamma$, and by the induction case for
      type we have $\kappa(\tr A) = A$, hence
      $\kappa(\tr(\Gamma,x:A)) = (\Gamma,x:A)$.
    \end{itemize}
  \item Types are either of the form $\Obj$ of or the form $\Hom{}tu$.
    \begin{itemize}
    \item For the type $\Obj$, we have $\tr \Obj = \Hom\Obj{x_0}{x_0}$
      and $\kappa\pa{\Hom\Obj{x_0}{x_0}} = \Obj$, hence
      $\kappa(\tr \Obj) = \Obj$.
    \item For a type of the form $\Hom Atu$, we have
      $\tr\pa{\Hom Atu} = \Hom{\tr A}{\tr t}{\tr u}$, and
      $\kappa\pa{\tr\pa{\Hom Atu}} = \Hom{\kappa(\tr A)}{\kappa(\tr
        t)}{\kappa(\tr u)}$. By the induction cases for types and
      terms, we have$ \kappa\pa{\tr\pa{\Hom Atu}} = \Hom Atu$.
    \end{itemize}
  \item Terms are either a variable or a coherence applied.
    \begin{itemize}
    \item For a term of the form of a variable $x$, $\tr x = x$ and
      $\kappa x = x$, thus $\kappa(\tr x) = x$.
    \item For a term which is an applied coherence
      $t = \coh_{\overline\Gamma,A}[\overline\sigma]$, we have
      \begin{align*}
        \tr t & =
                \pa{\coh_{\overline\Gamma,A}}^\sharp(\tr\overline\sigma)\\
        \kappa(\tr t) &=
                        \pa{\pa{\coh_{\overline\Gamma,A}}^\sharp}^\flat(\kappa^\sharp(\tr
                        \overline\sigma)).
      \end{align*}
      By the proposition~\ref{prop:flatten-fold} and the induction
      case for the substitutions to a monoidal ps-context, this proves
      \[
        \kappa\tr(\coh_{\overline\Gamma,A}(\overline\sigma)) =
        \coh_{\overline\Gamma,A}(\overline\sigma)
      \]
    \end{itemize}
  \item Substitutions are of the form $\sub{}$ or $\sub{\sigma,t}$.
    \begin{itemize}
    \item For the subsitution $\sub{}$, we have
      $\tr\sub{} = \sub{x_0}$ and $\kappa\sub{x_0} = \sub{}$ since
      $x_0$ is of dimension $0$. Hence $\kappa(\tr\sub{}) = \sub{}$.
    \item For a substitution of the form $\sub{\sigma,t}$, we have
      \begin{align*}
        \tr\sub{\sigma,t} &= \sub{\tr\sigma,\tr t} & 
                                                     \kappa\sub{\tr\sigma,\tr t} &= \sub{\kappa\tr\sigma,\kappa\tr t}      
      \end{align*}
      since necessarily $\dim(\tr t) > 0$. Hence, by induction case
      for the subsitutions and for the terms,
      $\kappa(\tr\sub{\sigma,t}) = \sub{\sigma,t}$.
    \end{itemize}
  \item A substitution to a monoidal ps-context is either $\bra{}$ or
    of the form $\bra{\overline\sigma,\tau}$.
    \begin{itemize}
    \item For the substitution $\bra{}$, we have
      $\tr(\bra{}) = \sub{x_0}$, and
      $\kappa^\sharp(\sub{x_0}) = \bra{}$, hence
      $ \kappa^\sharp(\tr \bra{}) = \bra{} $.
    \item For a substitution of the form $\bra{\overline\sigma,\tau}$,
      we have
      $\tr\bra{\overline\sigma,\tau} =
      \sub{\tr\overline\sigma,\tr\tau}$. Since $\tr{\tau}$ has to
      start with the variable $x_0$ of dimension $0$ and contains no
      other variable of dimension $0$, it follows that
      $\kappa(\sub{\tr\overline\sigma,\tr\tau}) =
      \bra{\kappa(\tr\overline\sigma);\kappa(\tr\tau)}$. By the
      induction case on substitution ot a monoidal ps-context and on substitution, we
      deduce that
      \[
        \kappa(\tr\overline\sigma) = \overline\sigma \qedhere
      \]
    \end{itemize}
  \end{itemize}
\end{proof}
\noindent In the converse direction, the result does not hold anymore,
intuitively, given a context $\Gamma$ in the theory $\CaTT$, the
context $\tr(\kappa \Gamma)$ is equal to the context $\Gamma$ where
all variables of dimension $0$ have been identified. The correct way
to formalize this intuition would be to use a most general unifier,
which in the case of this theory is a particular case of
equalizer\cite{catt-models}, however we will not need this
construction for proving our result of interest.

\subsection{Correctness}
Now that we have established translations between $\MCaTT$ and
$\CaTT$, we can prove the correctness of the type theory $\MCaTT$, \ie
its models are equivalent to the models of $\CaTT$ with only one
$0$-cell. While the definition of the translations merely formalized
the intuition behind $\MCaTT$, this part really justifies what makes
this intuition correct, by making these translations interact with the
structures of category with families of the syntactic categories on
each side.
\begin{lemma}
  Given a model $F : \Syn{\CaTT}\to\Set$, the functor induced by the
  pre-composition with $\tr$, $\tr^*(F) : \Syn{\MCaTT} \to \Set$
  defines a model of $\Syn{\MCaTT}$ if and only if $F$ is a
  $\omega$-category with only one $0$-cell (\ie $F$ is an object of
  $\OneObjCat$)
\end{lemma}
\begin{proof}
  Consider a model of $F : \Syn{\CaTT}\to \Set$ together with the
  induced functor $\iota ^* (F) : \Syn{\MCaTT} \to \Set$. By the
  proposition \ref{prop:almost-cwf-mor} and the note
  \ref{note:obstruction-terminal}, $\iota^* F$ may fail to be a model
  of $\Syn{\MCaTT}$ in only one way: it might not preserve the
  terminal object. All the rest of the structure of category with
  families is necessarily preserved by $\iota^*(F)$. This means that
  $\iota^*(F)$ is a model of $\Syn{\MCaTT}$ if and only if
  $\iota^*(F)(\emptycontext)$ is the terminal set
  $\set{\bullet}$. Note that
  $\iota^*(F)(\emptycontext) = F(\iota \emptycontext) = F(\D^0)$. So
  $\iota^*(F)$ is a model of $\Syn{\MCaTT}$ if and only if
  $F(\iota\D^0) = \set{\bullet}$, that is, by definition, if and only
  if $F$ is an object of $\OneObjCat$.
\end{proof}
\noindent In particular, this lemma implies that the functor $\iota$
induces a functor
\[
  \iota^* : \OneObjCat \to \Mod{\Syn{\MCaTT}}
\]



\begin{lemma}
  For any model of the theory $\MCaTT$, $F\in\Mod{\Syn{\MCaTT}}$, the
  induced functor $\kappa^*(F) : \Syn\CaTT \to \Set$ defines
  essentially uniquely a model of $\Syn\CaTT$.
\end{lemma}
\begin{proof}
  Since $\kappa$ preserves all the structure of category with families
  where it is defined, it is also the case for $\kappa^*(F)$. So it
  suffices to check that $\kappa^*(F)$ can be extended to transport
  all judgments in a unique way. In particular the only two kinds of
  judgments that cannot be transported through $\kappa$ are the ones
  of the form $\Gamma\vdash \Obj$ and $\Gamma\vdash t:\Obj$. Suppose
  that there is such a way to transport the type $\Obj$, then it has
  to satisfy
  \[
    \kappa^*(F)(\Gamma,x:\Obj) =
    (\kappa^*(F)(\Gamma),\kappa^*(F)(\Obj))
  \]
  Since $\kappa(\Gamma,x:\Obj) = \kappa\Gamma$, it follows that
  $\kappa^*(F) (\Gamma,x:\Obj) = \kappa^*(F)(\Gamma)$. On the other
  hand, $(\kappa^*(F)(\Gamma),\kappa^*(F)(\Obj))$ is obtained as the
  pullback
  \[
    \begin{tikzcd}
      (\kappa^*(F)(\Gamma),\kappa^*(F)(\Obj)) \ar[r]\ar[d]\ar[rd,phantom,"\lrcorner"very near start] & (\kappa^*(F)(\Obj))\ar[d]\\
      \kappa^*(F)(\Gamma)\ar[r] & \set{\bullet}
    \end{tikzcd}
  \]
  so $\kappa^*(F)(\Obj)$ has to satisfy the equation, for all context
  $\Gamma$,
  \[
    \kappa^*(F)(\Gamma) \times \kappa^*(F)(\Obj) \simeq
    \kappa^*(F)(\Gamma)
  \]
  This implies that $\kappa^*(F)(\Obj)$ has to be isomorphic to the
  singleton $\set{\bullet}$. Now we have to define an image for the
  term judgments of the form $\Gamma\vdash t:\Obj$. The image of such
  a judgment has to be an element of the type image of the judgment
  $\Gamma\vdash \Obj$, which is a singleton set $\set{\bullet}$, so
  there is no other choice than taking the unique element of the
  singleton. Conversely, extending $\kappa^*(F)$ with these images
  defines a morphism of category with families, as we designed them to
  be compatible with context extension and substitution extension.
\end{proof}
\noindent This lemma lets us consider $\kappa^*$ as a functor
$ \kappa^* : \Mod{\Syn{\MCaTT}} \to \Mod{\Syn{\CaTT}} $ and by
definition of $\kappa^*(F)$, we have that
$\kappa^*(F)(\D^0) = \set{\bullet}$, so in fact $\kappa^*$ corestricts
as
\[
  \kappa^* : \Mod{\Syn{\MCaTT}} \to \OneObjCat
\]

\begin{thm}
  The category of models of $\Syn\MCaTT$ is equivalent to the category
  $\OneObjCat$. More precisely the pair functors
  \[
    \begin{tikzcd}
      \OneObjCat \ar[r, shift left = 1, "\iota^*"] & \ar[l, shift left
      = 1, "\kappa^*"] \Mod{\Syn{\MCaTT}}
    \end{tikzcd}
  \]
  is an equivalence of categories.
\end{thm}
\begin{proof}
  Since $\kappa$ is a retract of $\iota$, it follows that
  $\iota^*\circ \kappa^* = \id{\Mod{\Syn{\MCaTT}}}$, so it suffices to
  show that conversely $\kappa^*\circ \iota^* =
  \id{\OneObjCat}$. Consider a category with only one object,
  $F \in \OneObjCat$, we show by induction on the length of $\Gamma $
  that $\kappa^*(\tr^* F) (\Gamma)$ is isomorphic to $F(\Gamma)$.
  \begin{itemize}
  \item If $\Gamma = \emptycontext$, and $\tr(\kappa\Gamma)$ is the
    context $(x_0 : \Obj)$ (disk of dimension $0$). Since
    $F \in \OneObjCat$, $F(\tr(\kappa\Gamma)) = \set{\bullet}$ is a
    singleton, and by definition of a model of $\Syn\CaTT$,
    $F(\emptycontext) = \set{\bullet}$ is also a singleton. Hence,
    $\kappa^*(\tr^* F) (\emptycontext)$ is isomorphic to
    $F(\emptycontext)$.
  \item If $\Gamma$ is of the form $(\Gamma',x:A)$ with $A$ distinct from the type $\Obj$, then
    $\kappa(\Gamma',x:A) = (\kappa\Gamma',x:\kappa A)$ and thus
    \[
      \tr(\kappa(\Gamma',x:A)) = (\tr(\kappa\Gamma'),\tr\kappa A)
    \]
    Hence, by induction hypothesis,
    \[
      F(\tr(\kappa(\Gamma',x:A))) = (F(\tr(\kappa \Gamma')),
      F(\tr(\kappa A))) \simeq (F(\Gamma'), F(A)) = F(\Gamma',x:A)
    \]
  \item If $A$ is the type $\Obj$, then
    $\kappa(\Gamma',x:\Obj) = \kappa(\Gamma')$ and
    $\tr(\kappa(\Gamma',x:\Obj)) = \tr(\kappa \Gamma')$, hence
    $F(\tr(\kappa (\Gamma',x:\Obj))) = F(\tr(\kappa \Gamma'))$. But on
    the other hand, the image
    $F(\Gamma',x:\Obj) = (F(\Gamma'),F(\Obj))$ is obtained as the
    following pullback
    \[
      \begin{tikzcd}
        F(\Gamma) \ar[r]\ar[d]\ar[rd,phantom,"\lrcorner" very near start] & F(\D^0)\ar[d] \\
        F(\Gamma') \ar[r] & F(\emptycontext)
      \end{tikzcd}
    \]
    Since $F$ is a category with only one object, this pullback
    rewrites as
    \[
      \begin{tikzcd}
        F(\Gamma) \ar[r]\ar[d]\ar[rd,phantom,"\lrcorner" very near start] & \set{\bullet}\ar[d] \\
        F(\Gamma') \ar[r] & \set{\bullet}
      \end{tikzcd}
    \]
    which shows that $F(\Gamma)$ is isomorphic to $F(\Gamma')$. Hence
    we have proved that in both cases, $F(\Gamma)$ is isomorphic to
    $F(\tr(\kappa \Gamma))$.\qedhere
  \end{itemize}
\end{proof}


==> monoidal.tex <==
\section{Type theory for monoidal weak $\omega$-category}
We now focus on monoidal categories. The idea here is to adapt the type theory
for weak $\omega$-categories, in order to enforce the constraint that our
categories should always have exactly one $0$-cell. To this end, we simulate the
existence of ``a virtual object of dimension $-1$'' in our monoidal
categories. There is no formal way in the theory for considering this object,
but all the rules act as if it existed.

\paragraph{The category of monoidal weak $\omega$-categories.}
Given a weak $\omega$-category $F$ in $\Mod{\Syn\CaTT}$, we call its
set of $0$-cells the image of the $0$-th dimensional disk
$F(\D^0)$. We thus denote $\OneObjCat$ the full subcategory of
$\Mod{\Syn{\CaTT}}$ whose objects are exactly the models $F$ of
$\CaTT$, such that $F(\D^0) = \set{\bullet}$.% The
% objects of this category are what we call the \emph{monoidal weak
% $\omega$-categories}.

\subsection{Lists of contexts}
In the theory $\CaTT$, the introduction rules for coherences relies on
the structure of ps-contexts. In the case of monoidal categories, we
have to adapt this structure, to what we call a \emph{monoidal
  ps-context}. Such a context is defined as a list of ps-contexts, the
intuition being that it is combinatorially equivalent to a single
ps-context, but with a shift of dimension. Let us illustrate this
correspondence with an example: Considering the following ps-context,
\[
  \begin{tikzpicture}[scale = 0.5]
    \coordinate (a) at (0,0); \coordinate (b) at (1,1); \coordinate
    (c) at (2,2); \coordinate (d) at (3,3); \coordinate (e) at (4,2);
    \coordinate (f) at (5,1); \coordinate (g) at (6,2); \coordinate
    (h) at (7,1); \coordinate (i) at (8,0); \coordinate (j) at (9,1);
    \coordinate (k) at (10,0); \coordinate (l) at (11,1); \coordinate
    (m) at (12,2); \coordinate (n) at (13,1); \coordinate (o) at
    (14,2); \coordinate (p) at (15,1); \coordinate (q) at (16,0);
      
      
    \draw (a)--(b); \draw (b)--(c); \draw (c)--(d); \draw (d)--(e);
    \draw (e)--(f); \draw (f)--(g); \draw (g)--(h); \draw (h)--(i);
    \draw (i)--(j); \draw (j)--(k); \draw (k)--(l); \draw (l)--(m);
    \draw (m)--(n); \draw (n)--(o); \draw (o)--(p); \draw (p)--(q);

      

    \fill (a) circle (0.1); \fill (b) circle (0.1); \fill (c) circle
    (0.1); \fill (d) circle (0.1); \fill (e) circle (0.1); \fill (f)
    circle (0.1); \fill (g) circle (0.1); \fill (h) circle (0.1);
    \fill (i) circle (0.1); \fill (j) circle (0.1); \fill (k) circle
    (0.1);\fill (l) circle (0.1); \fill (m) circle (0.1); \fill (n)
    circle (0.1); \fill (o) circle (0.1); \fill (p) circle (0.1);
    \fill (q) circle (0.1);
      

    \draw[thick] (-1,0)--(17,0);
  \end{tikzpicture}
\]
we shift its dimension by $-1$
\[
  \begin{tikzpicture}[scale = 0.5]
    \coordinate (a) at (0,0); \coordinate (b) at (1,1); \coordinate
    (c) at (2,2); \coordinate (d) at (3,3); \coordinate (e) at (4,2);
    \coordinate (f) at (5,1); \coordinate (g) at (6,2); \coordinate
    (h) at (7,1); \coordinate (i) at (8,0); \coordinate (j) at (9,1);
    \coordinate (k) at (10,0); \coordinate (l) at (11,1); \coordinate
    (m) at (12,2); \coordinate (n) at (13,1); \coordinate (o) at
    (14,2); \coordinate (p) at (15,1); \coordinate (q) at (16,0);
      
      
    \draw[dashed] (a)--(b); \draw (b)--(c); \draw (c)--(d); \draw
    (d)--(e); \draw (e)--(f); \draw (f)--(g); \draw (g)--(h);
    \draw[dashed] (h)--(i); \draw[dashed] (i)--(j); \draw[dashed]
    (j)--(k); \draw[dashed] (k)--(l); \draw (l)--(m); \draw (m)--(n);
    \draw (n)--(o); \draw (o)--(p); \draw[dashed] (p)--(q);

      

    \fill (a) circle (0.1); \fill (b) circle (0.1); \fill (c) circle
    (0.1); \fill (d) circle (0.1); \fill (e) circle (0.1); \fill (f)
    circle (0.1); \fill (g) circle (0.1); \fill (h) circle (0.1);
    \fill (i) circle (0.1); \fill (j) circle (0.1); \fill (k) circle
    (0.1);\fill (l) circle (0.1); \fill (m) circle (0.1); \fill (n)
    circle (0.1); \fill (o) circle (0.1); \fill (p) circle (0.1);
    \fill (q) circle (0.1);
      

    \draw[thick] (-1,1)--(17,1);
  \end{tikzpicture}
\]
and remove the $(-1)$-cells in order to finally obtain the following
list of ps-contexts
\[
  \begin{tikzpicture}[scale = 0.5]
    \coordinate (a) at (0,0); \coordinate (b) at (1,1); \coordinate
    (c) at (2,2); \coordinate (d) at (3,3); \coordinate (e) at (4,2);
    \coordinate (f) at (5,1); \coordinate (g) at (6,2); \coordinate
    (h) at (7,1); \coordinate (i) at (8,0); \coordinate (j) at (9,1);
    \coordinate (k) at (10,0); \coordinate (l) at (11,1); \coordinate
    (m) at (12,2); \coordinate (n) at (13,1); \coordinate (o) at
    (14,2); \coordinate (p) at (15,1); \coordinate (q) at (16,0);
      
      
    \draw (b)--(c); \draw (c)--(d); \draw (d)--(e); \draw (e)--(f);
    \draw (f)--(g); \draw (g)--(h); \draw (l)--(m); \draw (m)--(n);
    \draw (n)--(o); \draw (o)--(p);

      

    \fill (b) circle (0.1); \fill (c) circle (0.1); \fill (d) circle
    (0.1); \fill (e) circle (0.1); \fill (f) circle (0.1); \fill (g)
    circle (0.1); \fill (h) circle (0.1); \fill (j) circle (0.1);
    \fill (l) circle (0.1); \fill (m) circle (0.1); \fill (n) circle
    (0.1); \fill (o) circle (0.1); \fill (p) circle (0.1);

      

    \draw[thick] (0.5,1)--(7.5,1); \draw[thick] (8.5,1)--(9.5,1);
    \draw[thick] (10.5,1)--(15.5,1);
  \end{tikzpicture}
\]
Conversely, given a monoidal ps-context, there is a unique way to
assemble together all the elements of the list to produce a
ps-context. This is the intuition behind the type theory we introduce
for monoidal categories, and this intuition will be made formal via a
pair of translations between this theory and $\CaTT$ in
\secr{correctness}. Note that monoidal ps-contexts simulate many
virtual objects of dimensions $-1$, and not a single one, this will be
corrected later on, by only considering judgments in a regular
context.

\paragraph{Notations.}
For manipulating the lists, we always use overlined characters to
denote lists of the same type than the character, $\bra{}$ to denote
the empty list, and $\bra{\overline{a},b}$ to denote the list whose
tail is $\overline{a}$ and whose head is $b$. Moreover, given two
lists $\overline{a}$ and $\overline{b}$, we denote
$\overline{a}@\overline{b}$ their concatenation. Finally, for a list
$\overline{a}$, we denote $\ell(\overline{a})$ its length.


\paragraph{Monoidal ps-contexts.}
We introduce a new judgment to express the fact that a data is a
monoidal ps-context.
\[
  \begin{tabular}{c@{\quad : \quad}l}
    $\overline{\Gamma} \vdashps$ & $\Gbar$ is a well-formed monoidal ps-context \\[1.2ex]
  \end{tabular}
\]
The derivation rule for this judgment expresses that monoidal
ps-contexts are nothing more that a list of ps-contexts, with non
clashing variable names
\[
  \begin{array}{c@{\qquad\qquad\qquad\qquad}c}
    \inferrule{\null}{\bra{}\vdashps} & \inferrule{\Gbar\vdashps\\ \Delta\vdashps}{\bra{\Gbar;\Delta}\vdashps} \quad \pa{\Var\Delta \cap \Var\Gbar = \emptyset}
  \end{array}
\]
The monoidal ps-contexts come equipped with a notions of $i$-source,
by applying successively the $i$-source of ps-contexts to all its
elements.
\[
  \partial^-_i(\bra{}) = \bra{} \qquad\qquad\qquad\qquad
  \partial^-_i(\bra{\Gbar;\Gamma'}) = \bra{\partial^-_i\Gbar;
    \partial^-_i\Gamma'}
\]
This lets us define the general notion of source for monoidal
ps-contexts, which are useful for defining the introduction rules for
coherences
\[
  \partial^-\Gbar = \partial^-_{\dim \Gbar - 1} \Gbar
\]
Note that in the case of a monoidal ps-context of dimension $0$, (\ie
a list of ps-contexts all isomorphic to $\D^0$), this definition does
not make sense and we then use the convention that
$\partial^-\Gbar = \bra{}$. In general the case of the monoidal
ps-context of dimension $0$ is a limit case, and it will appear in
various places.  Similarly, monoidal ps-contexts come equipped with a
notion of target $\partial^+\Gbar$, defined the same way as the source from the
corresponding notion on ps-contexts. The following lemma is immediate
by definition of the source and the target,
\begin{lemma}
  \label{lemma:length-src-target}
  Any monoidal ps-context $\Gbar$ of dimension non $0$ has the same
  length than its source and its target
  $\ell(\Gbar) = \ell(\src\Gbar) = \ell(\tgt\Gbar)$.
\end{lemma}



\paragraph{Judgments for monoidal ps-contexts.}
Unlike the theory $\CaTT$, in this theory the monoidal ps-contexts are
not particular contexts (they are \emph{lists} of contexts) and
therefore we have to define a dedicated notion of type, term and
substitution in a ps-context. For this reason, we introduce new
dedicated judgments:
\[
  \begin{tabular}{c@{\quad : \quad}l}
    $\Gbar \vdash A$ & $A$ is a valid type in $\Gbar$ \\[1.2ex]
    $\Gbar \vdash t : A$ & $t$ is a valid term of type $A$ in $\Gbar$ \\[1.2ex]
    $\Gbar\vdash \sigma:\Delta$ & $\sigma$ is a valid substitution from $\Gbar$ to $\Delta$\\[1.2ex]
    $\Gbar\vdash \overline{\sigma} : \Dbar$ & The list $\overline{\sigma}$ is a valid  substitution from $\Gbar$ to $\overline{\Delta}$\\[1.2ex]
  \end{tabular}
\]
Note that even if the notation are similar, these judgments are
specific to the case where the left hand side is a monoidal
ps-contexts and should not be confused with the regular judgments of
our type theory. In particular, they are subject to the following
derivation rules, which provide a guarantee regarding the order in
which the ps-contexts of the list $\Gbar$ are used.
\[
  \begin{array}{c@{\qquad\qquad}c}
    \inferrule{\null}{\Gbar\vdash \Obj}
    &
      \inferrule{\Gbar\vdash
      t:A \\ \Gbar\vdash u:A}{\Gbar\vdash \Hom Atu} \\[2em]
    \inferrule{\Gbar\vdashps \\ \Gamma'\vdash t:A}{[\Gbar;\Gamma']\vdash t:A}
    &
      \inferrule{\overline\Gamma\vdash t:A  \\
    \Gamma'\vdashps}{\bra{\overline\Gamma;\Gamma'}\vdash t:A}\\[2em]
    \inferrule{\Gbar\vdashps}{\Gbar\vdash\sub{} : \emptycontext}
    &
      \inferrule{\Gbar\vdash \sigma:\Delta \\ \Delta\vdash A \\ \Gbar\vdash t:A[\sbar]}{\Gbar\vdash\sub{\sigma,t}:\Delta,x:A} \\[2em]
    \inferrule{\null}{\bra{}\vdash \bra{}:\bra{}}
    &
      \inferrule{\Gbar\vdash \sbar:\Dbar
    \\ \Gbar'\vdash \sigma' :
    \Delta' \\ \Delta'\vdashps}{\Gbar@\Gbar'\vdash\bra{\overline\sigma;\sigma'}
    : \bra{\Dbar;\Delta'}} 
  \end{array}
\]
% These rules are similar to the rules of $\CaTT$, and this is
% expected since they simulate the way derivations would happen in
% $\CaTT$, provided that the monoidal ps-context was a ps-context
% through the correspondence above. However, there is a major
% difference regarding substitutions, here our setup verifies that the
% variables of type $\Obj$ are ordered in the same way in a monoidal
% ps-context and in its associated substitution.
Imagining that the $0$-cells we are describing are in fact arrows over
objects of dimension $-1$, they come with an order and all derivable
terms, types and substitutions should respect this order. The rules we
just introduce are designed to enforce this order condition while
still never mentionning any dimension $-1$.


\paragraph{Categorical structure.}
There is a compoisition for substitutions between two monoidal
ps-context, as well as composition of such a substitution with a
substitution from a monoidal ps-context to a regular context. These
are defined mutually inductively as follows.
\[
  \begin{array}{c@{\qquad\qquad}c}
    \sub{}\circ \sbar = \sub{}
    &
      \sub{\tau,t}\circ\sbar =
      \sub{\tau\circ\sbar,t[\sbar]}\\[1.2em]
    \bra{} \circ \sbar = \bra{}
    &
      \bra{\overline\tau,\tau'}
      \circ\sbar = \bra{\overline\tau\circ\sbar;\tau'\circ\sbar}
  \end{array}
\]
Moreover, we also define the identity substitution between on monoidal
ps-context and itselft as the list constituted of only identity
substitutions. The composition previously defined is associative and
has the identity as left and right neutral element, this makes the
monoidal ps-contexts into a category, whith morphisms being the
monoidal substitutions.

\paragraph{Side conditions.}
Like in $\CaTT$, in order to derive coherences, we need to check side
conditions, and like in that case we encompass them into new
judgments.
\[
  \begin{tabular}{c@{\quad : \quad}l}
    $\Gbar \vdashop A$ & The type $A$ defines an admissible operation in $\Gbar$\\[1.2ex]
    $\Gbar \vdasheq A$ & The type $A$ defines an admissible equality in $\Gbar$ 
  \end{tabular}
\]
These judgments are very similar to those of the theory $\CaTT$ except
that they use our newly introduced judgments for monoidal ps-contexts
as premises, instead of regular judgments of the theory.  Besides, we
have to treat separately the case of the type $\Obj$, which has to be
made into an admissible operation, in order to describe the monoidal
product
\[
  \inferrule{\null}{\bra{\D^0}\vdashop \Obj} \qquad\qquad
  \inferrule{\Gbar\vdashop\Obj}{\bra{\Gbar;\D^0}\vdashop \Obj}
\]
\[
  \inferrule{\Gbar\vdashps \\ \src\Gbar\vdash t : A \\
    \tgt\Gbar\vdash u:A}{\Gbar\vdashop \Hom Atu} \quad \left\{
    \begin{array}{l}
      \Var{t:A} = \Var{\src\Gbar}\\
      \Var{u:A} = \Var{\tgt\Gbar}
    \end{array}
  \right.
\]
\[
  \inferrule{\Gbar\vdashps \\ \Gbar\vdash A}{\Gbar\vdasheq A}\quad\Var
  A = \Var\Gbar
\]


\paragraph{Coherences.}
We now introduce a term constructor $\coh$, whose arguments are a
monoidal ps-context, a type and a substitution between moniodal ps-contexts. We denote the
term $\coh_{\overline{\Delta},A}[\overline{\sigma}]$. The introduction
rules for such terms are the two following ones
\[
  \begin{array}{c@{\qquad\qquad}c}
    \inferrule{\Dbar\vdashop A \\ \Gbar\vdash \sbar:\Dbar}
    {\Gbar\vdash\coh_{\Dbar,A}(\sbar) : A[\sbar]}
    &
      \inferrule{\Dbar\vdasheq A \\
    \Gbar\vdash\sbar:\Dbar}{\Gbar\vdash \coh_{\Dbar,A}(\sbar) :
    A[\sbar]}
    
  \end{array}
\]
Where the notation $A[\sbar]$ (\resp $t[\sbar]$) is the application of
the monoidal substiution $\sbar$ to the type $A$ (\resp to the term
$t$), defined by induction a follows
\[
  \begin{array}{r@{\quad\equiv\quad}l}
    \Obj [\sbar] & \Obj \\
    \par{\Hom Atu} [\sbar] & \Hom {A[\sbar]}{t[\sbar]}{u[\sbar]}
  \end{array}
  \qquad
  \begin{array}{r@{\quad\equiv\quad}l}
    \coh_{\Gbar,A} (\overline{\gamma})[\sbar] & \coh_{\Gbar,A}(\overline{\gamma}\circ\sbar)
  \end{array}
\]
Note that with these definitions for coherences and for applying
monoidal substitutions, the following rules are admissible. These rule
express a compatibility between application of the substitution and
the typing rules.
\[
  \inferrule{\Gbar\vdashps \\ \Gbar\vdash A \\ \Dbar\vdash \sbar :
    \Gbar}{\Dbar\vdash A[\sbar] } \qquad \inferrule{\Gbar\vdashps \\
    \Gbar\vdash t:A \\ \Dbar\vdash \sbar : \Gbar}{\Dbar \vdash
    t[\sbar] : A[\sbar]}
\]




\subsection{The type theory $\MCaTT$}
Up until now, the system that we have presented is incomplete, as it
only adds judgments whose left hand side is a monoidal
ps-contexts. Those judgments are not part of the structure of type
theory, hence they do not change the models. Moreover, we had
announced that we want to simulate a single object in dimension $-1$,
and we presented a system that simulates many of them. In order to fix
this, we present a way to derive regular judgments from these new
judgments we have introduced. This requires the use of a new kind of
substitution going from a regular context to a monoidal ps-context,
and which plays two roles. Firstly it allows for judgments in a
monoidal ps-context to generate judgments in regular contexts, which
has an effect on the models of the theory, and secondly it ensures
that all the virtual objects of dimension $-1$ that were simulated in
monoidal ps-contexts get (virtually) sent onto a unique virtual object
of dimension $-1$ simulated in a regular context.


% Up until now, the system we have presented is not very powerful. It
% allows for the definition of some terms in monoidal ps-contexts, but
% in fact very few of them. This is because to produce new terms in
% monoidal ps-contexts, we need to provide subsitutions between them
% which are defined using the usual subsitutions between contexts. But
% the theory does not have any terms in the contexts yet, except for
% the variables, so ther are very few such substitutions. To fix this,
% we introduce a new kind of substitutions, which connect a context to
% a monoidal ps-context, along with an operation of applying such a
% substitutions to transfer terms in the monoidal ps-context to terms
% in the context. The resulting type theory is called $\MCaTT$.

\paragraph{Substitutions to a monoidal ps-context.}
In order to build a bridge between the world of monoidal ps-context
and our type theory, and transfer our newly introduced terms built out
of coherences to a regular context, we need to introduce a new sort of
substitution, that goes from a regular context to a monoidal
ps-context. These substitution are characterized by the following
judgment:
\[
  \begin{tabular}{c@{\quad : \quad}c}
    $\Delta \vdash \sbar : \Gbar$ & $\sbar$ is a well-formed substitution from $\Delta$ to $\Gbar$
  \end{tabular}
\]
As the notation suggests, these substitutions are supported by lists
of susbtitutions, and the derivation rules to which they are subject
are the following
\[
  \inferrule{\Delta\vdash}{\Delta\vdash \bra{} : \bra{}} \qquad
  \inferrule{\Delta\vdash\sbar:\Gbar \\
    \Delta\vdash\sigma':\Gamma'}{\Delta\vdash \bra{\sbar;\sigma'} :
    \bra{\Gbar;\Gamma'}}
\]
Note that such subsitution compose on the right with the usual
subsitutions, and on the left with the substitutions from a monoidal
ps-context. These compositions are associative and given by the
following formulas
\[
  \begin{array}{c@{\qquad}c}
    \bra{} \circ \gamma \equiv \bra{}
    &
      \bra{\sbar;\sigma'}\circ\gamma \equiv \bra{\sbar\circ\gamma;\sigma'\circ\gamma}\\[1.2em]
    \sub{}\circ\sbar\equiv \sub{}
    &
      \sub{\gamma,t}\circ\sbar\equiv \sub{\gamma\circ\sbar,t[\sbar]}\\[1.2em]
    \bra{} \circ \sbar \equiv \bra{}
    &                             
      \bra{\overline\gamma;\gamma'}\circ\sbar\equiv\bra{\overline\gamma\circ\sbar;\gamma'\circ\sbar}
  \end{array}
\]
By orienting these relations left to right, it provides a confluent
rewriting system for such substitutions, which gives an algorithm
deciding whether two such substitutions are equal or not.

\paragraph{Defining terms in general contexts.}
We now use this new kind of substitutions to define terms and types in
regular contexts from terms and types derived in monoidal
ps-contexts. This is achieved by two new type constructors $t[\sbar]$
and $A[\sbar]$, along with the following introduction rules
\[
  \inferrule{\Gbar\vdashps \\ \Gbar\vdash A \\ \Delta\vdash \sbar :
    \Gbar}{\Delta\vdash A[\sbar] } \qquad \inferrule{\Gbar\vdashps \\
    \Gbar\vdash t:A \\ \Delta\vdash \sbar : \Gbar}{\Delta\vdash
    t[\sbar] : A[\sbar]}
\]
This introduces too many terms that representing the same operation,
so in order to reduce the number of derivable terms to the minimum, we
need to quotient by some relations, expressing the compatibility of
type formers and term formers with the substitution operations.
\[
  \begin{array}{r@{\quad\equiv\quad}l}
    \Obj[\sbar]
    & \Obj \\
    \par{\Hom Atu} [\sbar]
    & \Hom {A[\sbar]}{t[\sbar]}{u[\sbar]}
  \end{array}
  \qquad
  \begin{array}{r@{\quad\equiv\quad}l}
    \coh_{\Gbar,A}(\sbar)[\gamma]
    & \coh_{\Gbar,A}(\sbar\circ\gamma) \\
    \coh_{\Gbar,A}(\overline{\gamma})[\sbar]
    & \coh_{\Gbar,A}(\overline{\gamma} \circ \sbar) 
  \end{array}  
\]
By orienting these relations left to right as they are written, they
define a confluent rewriting system, thus providing with an algorithm
for type checking.

\paragraph{Coherences.} The above rewriting rules give normal forms
for terms which are not variables, of the form
\[
  \Delta\vdash \coh_{\Gbar,A}(\sbar) : A[\sbar]
\]
for a substitution $\sbar$ going from a context to a monoidal
ps-context. In order to simplify our syntax, we introduce
\emph{coherences}, that are terms of the form (implicitly taking as
argument an identity substitution)
\[
  \Gbar\vdash \coh_{\Gbar,A} : A
\]
Then our rewriting system shows that all terms are obtained by applying a substitution
to such a coherence.


\subsection{Examples of derivations}
Here are few examples and counter-exmaple of derivable terms in
$\MCaTT$, to illustrate how they describe monoidal weak
$\omega$-categories.
\begin{itemize}
\item Monoidal product: we can define the monoidal tensor product in
  $\MCaTT$ as the coherence
  \[
    \texttt{prod} := \coh_{\bra{(x:\Obj);(y:\Obj)},\Obj} 
  \]
  By composing with a substitution, for every objects $t$ and $u$ (of
  type $\Obj$) in a given context~$\Gamma$, we can form their tensor
  product as
  \[
    \Gamma\vdash\texttt{prod}\ t\ u : \Obj
  \]
  % This coherence lets us derive a term witnessing the existence of
  % monoidal product in a context containing at least two objects, by
  % pulling back along a substitution towards the list
  % $\bra{(x:\Obj);(y:\Obj)}$
  % \[
  %   (x : \Obj, y : \Obj) \vdash \texttt{prod}\ x\ y : \Obj
  % \]
\item Associativity of monoidal product: similarly, we can define the
  valid coherence
  \[
    \texttt{assoc} :=
    \coh_{\bra{(x:\Obj);(y:\Obj);(z:\Obj)},\Hom{}{\texttt{prod}\ x\
        (\texttt{prod}\ y\ z)}{\texttt{prod}\ (\texttt{prod}\ x\ y)\
        z}}
  \]
  Using this coherence, for every object $t,u$ and $v$ (of type
  $\Obj$) in a given context~$\Gamma$, we can form a witness of
  associativity
  \[
    \Gamma \vdash \texttt{assoc}\ t\ u\ v : \Hom \Obj {\texttt{prod}\
      t\ (\texttt{prod}\ u\ v)} {\texttt{prod}\ (\texttt{prod}\ t\ u)\
      v}
  \]
\item Neutral element: it is also possible to derive the neutral
  element for the monoidal product, which can be viewed as a nullary
  monoidal product. It is defined as a coherence
  \[
    \texttt{e} := \coh_{\bra{},\Obj}
  \]
  In any context, one compose with the empty substitution, in order to
  get the term witnessing the neutral element.
  \[
    \Gamma\vdash \texttt{e} \bra{} : \Obj
  \]
  In order to simplify the notations, we may simply denote
  $\texttt{e}$ in any context, and omit the empty substitutions
  $\bra{}$ which carries no information.
\item Cancellation witness: one can also prove in $\MCaTT$ that the
  term $\texttt{e}$ is indeed a neutral element for the monoidal
  product, here for instance on the left. This is done by the
  coherence
  \[
    \texttt{l-unit} := \coh_{\bra{(x:\Obj)},\Hom{}{(\texttt{prod}\
        \texttt{e} \ x)}{x} }
  \]
  This coherence can be used to derive, for eny object $u$ in a
  context $\Gamma$, the following witness of left unitality of
  $\texttt{e}$
  \[
    \Gamma \vdash \texttt{l-unit}\ u : \Hom{}{(\texttt{prod}\
      \texttt{e}\ u)}{u}
  \]
\item Functoriality of monoidal product: The following coherence
  defines the functoirality for monoidal product
  \[
    \texttt{funl} :=
    \coh_{\bra{(x:\Obj,y:\Obj,f:\Hom{}xy);(z:\Obj)},\Hom{}{(\texttt{prod}\
        x\ z)}{(\texttt{prod}\ y\ z)}}
  \]
  Given any three objects $u,u',v$ together with a term $t$ of type
  $\Hom{}u{u'}$ in a context $\Gamma$, this coherence can be used to
  derive a witness for the fonctoriality of the monoidal tensor
  product on the left
  \[
    \Gamma \vdash \texttt{funl}\ t\ v : \Hom{}{(\texttt{prod}\ u\
      v)}{(\texttt{prod}\ u'\ v)}
  \]
\item Symmetry of the monoidal product: note that the same idea does
  not apply to derive the symmetry of the monoidal product. Indeed, if
  we try to build a witness for symmetry, it would be a term
  \[
    \texttt{sym} :=
    \coh_{\bra{(x:\Obj);(y:\Obj)},\Hom{}{\texttt{prod}\ x\ y}
      {\texttt{prod}\ y\ x}}
  \]
  It turns out that the list
  $\bra{(x:\Obj);(y:\Obj)} \vdash \bra{\sub{y};\sub{x}} : \bra{(x :
    \Obj);(y:\Obj)}$ is not a valid substitution, which makes the
  judgment $\bra{(x:\Obj);(y;\Obj)}\vdash \texttt{prod}\ y\ x$ not
  derivable. So the term $\texttt{sym}$ is not derivable in
  $\MCaTT$. This is a safety check, since the internal language for
  monoidal categories is supposed to be unable to derive a witness for
  commutativity.

\end{itemize}



